Regret-Minimization Algorithms for Multi-Agent Cooperative Learning Systems

A Multi-Agent Cooperative Learning (MACL) system is an artificial intelligence (AI) system where multiple learning agents work together to complete a common task. Recent empirical success of MACL systems in various domains (e.g. traffic control, cloud computing, robotics) has sparked active research into the design and analysis of MACL systems for sequential decision making problems. One important metric of the learning algorithm for decision making problems is its regret, i.e. the difference between the highest achievable reward and the actual reward that the algorithm gains. The design and development of a MACL system with low-regret learning algorithms can create huge economic values. In this thesis, I analyze MACL systems for different sequential decision making problems. Concretely, the Chapter 3 and 4 investigate the cooperative multi-agent multi-armed bandit problems, with full-information or bandit feedback, in which multiple learning agents can exchange their information through a communication network and the agents can only observe the rewards of the actions they choose. Chapter 5 considers the communication-regret trade-off for online convex optimization in the distributed setting. Chapter 6 discusses how to form high-productive teams for agents based on their unknown but fixed types using adaptive incremental matchings. For the above problems, I present the regret lower bounds for feasible learning algorithms and provide the efficient algorithms to achieve this bound. The regret bounds I present in Chapter 3, 4 and 5 quantify how the regret depends on the connectivity of the communication network and the communication delay, thus giving useful guidance on design of the communication protocol in MACL systems

==> greedybayes.tex <==

\section*{\textbf{\Large{Chapter 6}}}
\addcontentsline{toc}{section}{Chapter 6.  The Sequential Learning of Maximum-Valued Matching}

\bigskip
\bigskip

\textbf{\Large{The Sequential Learning of Maximum Value Matching}}

\bigskip
\bigskip
\bigskip

\noindent{
Efficiently finding a maximum value matching for a given set of nodes based on observations of values of matches over a sequence of rounds is a fundamental sequential learning problem. Here a matching refers to a set of matches of node pairs (or matches in short) such that each node is matched to at most one other node. This problem arises in many applications including team formation, online social networks, online gaming, online labor, and other online platforms. We may think of the nodes as agents in MACL systems and the value of a matched node pair to represent the reward or welfare generated from interaction or joint production of the two agents, contributing to the total reward or welfare. For example, in team production, the value of a matched pair of nodes may represent the quality of the work produced. In online social networks, the value of a matched pair of nodes may represent user satisfaction or social capital gained through interaction. 
}

\subsection{Introduction}



We consider the case when the value of each matched pair of nodes is according to a function -- we refer to as a value function -- of latent node features in some domain. We focus on the case of a finite domain such that each node is either of low or high type, which can be represented by each node having value $0$ or $1$ -- we refer to this as latent binary types. For value functions, we consider all symmetric Boolean functions, as well as a popular production function used in economics literature known as Constant Elasticity of Substitution (CES). The types of nodes are a priori unknown and partial information about node types is acquired as values of matches are observed. The underlying value function plays a key role in how much information is revealed about individual node types from observed values of matches. For example, for Boolean OR function, having observed value of a match to be $0$, we can immediately deduce that both nodes are of low type, and, otherwise, the only conclusion that can be drawn is that at least one node is of high type. The decision maker gains partial information about individual node types as outcomes of matches are observed over a sequence of rounds. We consider this decision problem under the constraint that sequence of matchings must be incremental, meaning that in each round the selected matching is derived by a limited change of the matching in the previous round. Specifically, we consider the case when in each round the decision maker can only choose a matching that is identical to the matching selected in the previous round, except for possibly re-matching any two previously matched pairs. Learning how to match through an incremental sequence of matchings limits how much information can be gained about individual node types in each round. This constraint is motivated by applications in practice when matched node pairs remain matched over several rounds, allowing only a small change of matching to be made in each round. 

We consider the underlying incremental matching problem for a set of $n$ nodes in a Bayesian setting where latent binary types of nodes are according to a prior product-form Bernoulli distribution with parameter $p$. Here $p$ is the probability that a node is of high type according to the prior distribution. We study greedy Bayes incremental matching strategies that in each round select a matching that has highest marginal value from the set of feasible matchings (obeying incremental matching constraint), according to posterior distribution, given the information observed up to the current round. We evaluate performance of greedy Bayes incremental matching strategies by considering expected Bayesian regret, defined as the difference between cumulative expected value of an optimal matching and expected value of the sequence of matchings chosen by the algorithm asymptotically for large number of rounds. Our goals are to identify greedy Bayes incremental matching strategies for different value functions, and characterize expected Bayesian regret under different value functions.  


\subsubsection{Related work}

Team formation problems were studied under various assumptions in different scientific fields and application domains. \cite{KM18}, \cite{SVY20}, \cite{ts-dabeen} and \cite{notes} studied individual skill scoring methods for the best team selection, or assigning individuals to teams, for various functions determining team performance from individual performances. \cite{NWN99} studied the relationship between work team effectiveness and two aspects of the personality traits of team members, namely, the average level of a given trait within a team, and the variability in traits within a team. \cite{CE10} studied the problem of formations of teams through a pricing mechanism, where individuals are partitioned into groups of equal size and each team requires exactly one member from each group. When there are two groups, the problem corresponds to the classic marriage problem. \cite{liemhetcharat} studied the team formation problem where each individual has its own capabilities and the performance of a team depends on capabilities of team members as well their pairwise synergies. \cite{RMKT17} studied the problem of partitioning individuals into disjoint groups for different objectives that account for pairwise compatibility of individuals. \cite{FT20} studied the problem of inferring individual from team productivity using a scoring method leveraging varying membership and level of success of all teams. Popular skill rating systems used in online gaming platforms, such as TrueSkill, assume team performances to be sum of individual performances with some added noise, and matching strategies are used aiming to match players of similar skills in order to make interesting competitions \cite{GMH07}. 

The most closely related work to ours is \cite{johari18} which introduced the problem of incremental matching with match outcomes according to a function of binary latent types. They considered regret for maximum value and minimum value functions. For maximum value (Boolean OR) function, their 1-chain algorithm is a greedy Bayes incremental matching algorithm, for which we show a tight regret characterization. For minimum value (Boolean AND), they studied an algorithm and established some comparison results. Our work identifies the greedy Bayes incremental matching algorithm and establishes a regret bound. Our work further extends this work in identifying greedy Bayes incremental matching strategies and analysing regret for all symmetric Boolean value functions, as well as CES value function. \cite{synergy} studied the same problem, but without the constraint that the sequence of matchings must be according to an incremental matching sequence. They established tight regret bounds for all symmetric Boolean value functions. 

The problem we consider has some connections with combinatorial bandits that have been studied under various assumptions, e.g. \cite{comb}, \cite{CTPL15}, \cite{KZAC15}, \cite{combgenreward}, \cite{combsumfull}, \cite{combstochdom}. For combinatorial bandits, in each round, the decision maker selects an arm that corresponds to a feasible subset of base arms. For example, given a set of $N$ base arms, an arm is an arbitrary subset of base arms of cardinality $K$. Under full bandit feedback, the reward of the selected arm is observed, which is according to an underlying function of the  corresponding base arms' values. For example, this may be sum of values \cite{comb,CTPL15,combsumfull}, or some non-linear function of values (such as maximum value) \cite{combgenreward,combstochdom}. Under semi-bandit feedback, individual values of all selected base arms are observed. In our setting, we may think of node pairs to be base arms, matchings to be arms, and we have semi-bandit feedback. Alternatively, we may regard nodes to be base arms, matchings to be arms, and we have full-bandit feedback for each match in a matching. Note that requiring for sequence of matching selections to be according to an incremental matching sequence is not studied in the line of work on combinatorial bandits. 

\cite{SKB16} studied the best-of-$K$ bandit problem in which at each time step, the decision maker chooses a subset of $K$ arms from a set of $N$ arms and observers reward equal to maximum of individual arm's values drawn from a joint distribution. Here the objective is to identify the subset that achieves the highest expected reward using as few queries as possible. 

Regret minimization for maximum weight matching problems with stochastic edge weights whose mean values obey a rank-1 structure was studied in \cite{flore}. Here the mean weight $w_{u,v}$ for two nodes $u$ and $v$ is of the form $w_{u,v} = \theta_u \theta_v$, where $\theta_1, \ldots, \theta_n$ are hidden node parameters with values in $[0,1]$. The stochastic weight of an edge is defined as the sum of mean edge weight and a sub-Gaussian random noise. An adaptive matching algorithm is shown to have regret of order $n\log(T)$ up to a poly-logarithmic factor. Note that the rank-1 assumption along with assuming that node parameters are binary and zero noise boil, down to weights according to Boolean OR function. Our work is different in that we consider noiseless weights, binary node types, and we admit the incremental matchings constraint.   

Another related line of work is on group testing, which is about detection of nodes in state $1$ in a population of nodes with each node being in either state $0$ or $1$, by using group tests; e.g. by \cite{AS12}, \cite{MN14}, \cite{CJBJ17}. Each outcome of a group test is according to Boolean OR function of individual node states corrupted with some noise. The objective is to identify all nodes in state $1$ with a minimum number of group tests, where each group test is allowed to be performed on an arbitrary subset of nodes. The main difference with our setting is in that we restrict each group test to be for a pair of nodes, pair tests must be performed simultaneously in each round according to a matching, and successive matchings must obey the incremental matching constraint. In addition, our focus is on regret minimization, not sampling complexity. 

Finally, our problem bears some similarity with identification of latent node types from observed edge values for different random graph models. For stochastic block models \cite{holland} (see also survey of recent results \cite{abbe}), a basic model is for a set of nodes with binary latent types with independent Bernoulli edge outcomes with probability $p$ for a candidate edge between two nodes of same type and $q < p$ for a candidate edge between two nodes of different types. The goal is to accurately cluster nodes with respect to their latent types. \cite{GRSY15} considered the problem of inferring latent node types, which take values $-1$ or $1$, based on values of edges of a fixed graph. Each edge has value $1$ for two nodes of the same type, and value $-1$ for two nodes of different types, corrupted with a random sign-flip noise. These edge values of these random graph models could be seen to be akin to a negated XOR value function. Other work concerned with inferring latent node parameters from observed edge outcomes is for $\beta$-model random graphs \cite{chatterjee2011}, \cite{rinaldo}, \cite{MMS18}, where an edge exists between a pair of two candidate nodes with probability proportional to a logistic function of the sum of the latent parameter values of the two nodes. 

% \subsubsection{Summary of our contributions}

% We identified greedy Bayes incremental matching strategies for all symmetric Boolean and CES value functions. For some value functions, greedy Bayes incremental matching amounts to an interesting dynamics of matching sets, representing posterior beliefs, which are merged or dissolved upon exploring matches spanning two matching sets. For example, this arises for minimum (Boolean AND) and dissimilarity (Boolean XOR) value functions. 

% We established lower bounds on regret for each value function that hold for any adaptive matching algorithm, which depend on $n$ and $p$. For any fixed value $p$, these lower bounds scale quadratically with the number of nodes $n$. For value functions under which greedy Bayes incremental matching satisfies a constant improvement property, the greedy Bayes incremental matching has regret upper bound matching the lower bound up to a constant factor. The constant improvement property holds under affinity (negated XOR) and CES value functions. 

% We established upper bounds on regret for greedy Bayes incremental matching algorithms for different value functions. All these bounds scale quadratically with the number of nodes $n$, for fixed value of parameter $p$. The scaling of regret with $p$ can be different for different value functions. For some value functions, the regret of greedy Bayes incremental matching algorithm achieves highest values for $p=1/2$ and it symmetrically decreases as $p$ is further away from $1/2$. For example, this is the case for affinity (negated XOR) value function and CES value function. 

% For maximum (Boolean OR) value function, the regret scales as $((2-p)/p)\min\{p,1-p\}^4 n^2$. Hence, it scales proportionally to $p^3 n^2$, for small $p$, and proportionally to $(1-p)^4 n ^2$, for large $p$. This shows that the case of rare high-type nodes is harder than the case of rare low-type nodes. This is intuitive as a positive value for a match is realised only if at least one of the matched nodes is a high-type node. 

% For CES value functions, the regret crucially depends on whether the value function corresponds to substitutes ($0 < a \leq 1$) or complements ($a > 1$). For the case of complements, the regret is proportional to $\min\{p, 1-p\}^4 n^2$, for large $n$. The extra feedback, in comparison with maximum (Boolean OR) value function, amounts to a smaller regret with respect to dependence on parameter $p$. For the case of substitutes, the regret scales as $(p(1-p))^2 n^2$, for large $n$, which is worse than for complements in the regimes when either type of nodes is rare.  

% For minimum (Boolean AND) and dissimilarity (Boolean XOR) value functions, the state evolution under greedy incremental matching involves a collection of matching sets whose analysis is somewhat intricate. In this case, we provide some bounds and test them with numerical experiments. Perhaps interestingly, for minimum (Boolean AND) value function, the regret sharply increases with $p$ from $p=0$ to a maximum value, and then decreases to zero at $p=1$. The rarer the high-type nodes are, the more difficult is to find a match consisting of two high-types nodes, and, hence, as a result, the higher the regret.  

\subsubsection{Organization of this chapter}

In Section~\ref{sec:problem} we present problem formulation and notation used in the paper. Section~\ref{sec:results} contain our results, starting with a regret lower bound, and then showing greedy Bayes incremental matching algorithm and its analysis for each value function studied separately in different subsections. In Section~\ref{sec:conc} we state concluding remarks. Appendix contains proofs for theorems stated in the paper. 

\subsection{Problem formulation}
\label{sec:problem}

Let $V = \{1,\ldots, n\}$ be a set of $n$ nodes, where $n$ is an even, positive integer. Each node $v\in V$ has a latent variable $\theta_v$ that takes value in $\Theta = \{0, 1\}$. We refer to the latent variable of a node as the \emph{type} of node. Type $0$ is referred to as \emph{low type} and type $1$ is referred to as  \emph{high type}.

The latent variables $\theta = (\theta_1, \ldots, \theta_n)$ are assumed to have a prior distribution of product-form with identical Bernoulli marginal distributions, i.e. $\P[\theta_v = 1] =1-\P[\theta_v = 0]= p$, for all $v\in V$, for some $p \in [0,1]$. Intuitively, parameter $p$ characterises the population of nodes with respect to their types--we may think of as the portion of high-type nodes in the population. 

Each match of a pair of nodes $(u,v)$, has \emph{weight} $w_{u,v} = \f(\theta_u, \theta_v)$ where $\f$ is a symmetric function $\f: \Theta^2 \rightarrow \tilde{\Theta}$. A function is said to be symmetric if its output is invariant to permutations of its inputs. Set $\tilde{\Theta}$ is assumed to be fixed---its elements do not depend on either $n$ or $p$. We refer to $\f$ as a \emph{value function}, quantifying the value of a pair of nodes. When $\tilde{\Theta} = \{0,1\}$, then $\f$ is a Boolean function. We consider all symmetric Boolean functions with dual input, which are defined as follows:
\begin{itemize}
    \item Null: always 0
    \item Identity: always 1
    \item AND: $1$ if both inputs are $1$, otherwise $0$
    \item NAND: $0$ if both inputs are $1$, otherwise $1$
    \item OR: $0$ if both inputs are $0$, otherwise $1$
    \item NOR: $1$ if both inputs are $0$, otherwise $0$
    \item XOR: $1$ if either input is $1$, but not both (in other words, $1$ if inputs are different)
    \item NXOR: $1$ if inputs are equal, otherwise $0$.
\end{itemize}

Clearly, Null and Identity are of no interest, as there is a trivial matching solution under either of these two value functions which has zero regret. Hence, we are left with six symmetric Boolean functions for consideration. 

For any two Boolean functions $\f$ and $\bar{\f}$, we say that they are input-negated equivalent, if $\bar{\f}$ has same outputs as by applying $\f$ to negated inputs of $\bar{\f}$, i.e. $\bar{\f}(x,y)=\f(\neg x, \neg y)$, or vice versa. AND and NOR are input-negated equivalent, OR and NAND are input-negated equivalent, while XOR is input-negated equivalent to itself, and NXOR is input-negated equivalent to itself.  Any adaptive matching algorithm has the same regret for two input-negated equivalent functions. It follows that to study regret for all symmetric Boolean value functions, it suffices to consider AND, OR, XOR, and NXOR value functions.  

We refer to Boolean OR as \emph{maximum} value function, Boolean AND as \emph{minimum} value function, Boolean XOR as \emph{dissimilarity} value function, and Boolean NXOR as \emph{affinity} value function. 

In addition, to symmetric Boolean value functions, we also consider a function defined as $\f(x,y)=(x^a+y^a)^{1/a}$, for parameter $a > 0$. Functions of this form are studied as production functions in economics literature where they are referred to as Constant Elasticity of Substitution (CES) functions. The case when $0 < a\leq 1$ is referred to as substitutes and case $a>1$ is referred to as complements. Note that for Boolean inputs, the output of a CES function with parameter $a$ is $0$ for input $(0,0)$, $1$ for input either $(0,1)$ or $(1,0)$, and $2^{1/a}$ for input $(1,1)$. In comparison to maximum (Boolean OR) value function, the output is more informative only for the input $(1,1)$, allowing to distinguish when two nodes are of different type or are both of high type. 

These value functions are natural choices and have been studied in the context of production systems. Boolean OR value function requires at least one node of a pair of nodes to be of high type for the value of the pair to be high. In other words, the value of a pair is the value of the highest type node of this pair. This function is sometimes referred to as \emph{strongest link} function. The CES function allows for different definitions of the value of a pair for different values of parameter $a$. In the limit as $a\downarrow 0$, the value of a pair is equal to the sum of individual node values. In the other extreme, as $a$ goes to infinity, the value of a pair is the maximum value of individual nodes. Boolean AND value function requires both nodes of a pair of nodes to be of high type for the value of the pair to be high. This value function is sometimes referred to as the \emph{weakest link} function, indicating that the value of a pair of nodes is the value of the lowest type node of this pair. 

The value $w_{u,v} =\f(\theta_u,\theta_v)$ of a pair of nodes $(u,v)$ may only reveal a \emph{partial information} about values of node types $\theta_u$ and $\theta_v$. We discuss this for functions $\f$ that we consider as follows. For Boolean OR value function, if $w_{u,v} = 0$, then we can deduce that \emph{both} $u$ and $v$ are of low type, and, otherwise, if $w_{u,v} = 1$, then we can deduce that \emph{either} $u$ or $v$ is of high type. For a CES function, there are three possible output values. If $w_{u,v}=0$, then we can deduce that both $u$ and $v$ are of low type, if $w_{u,v}=1$, then we can deduce that $u$ and $v$ are of different types (one is of high and the other is of low type), and, finally, if $w_{u,v}=2^{1/a}$, then both $u$ and $v$ are of high type. Observe that a CES value function reveals more information about node types than Boolean OR value function. For a CES function, we can exactly detect whether or not nodes are of different types, and the only remaining uncertainty is when nodes are of different types. On the other hand, for Boolean OR value function we can exactly detect whether or not both nodes are of low type, and there is a remaining uncertainty for all other combinations of node types. For minimum (Boolean AND) value function, if $w_{u,v}=0$, then we can deduce that \emph{either} $u$ or $v$ is of low type, and , otherwise, if $w_{u,v}=1$, then we can deduce that \emph{both} $u$ and $v$ are of high type. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=14cm]{inc-match.pdf}
\caption{An example of an incremental matching sequence: for example, the second matching is derived from the first matching by re-matching node pairs $(2,3)$ and $(4,5)$.}
\label{fig:inc-match}
\end{center}
\end{figure}


We consider the problem of finding a maximum value matching of nodes in a sequential decision making setting. An adaptive matching algorithm $\alg$ selects a matching $M_t^{\alg}$ in each round $t = 1, \ldots,T$ from a set of \emph{permissible matchings} $\mathcal{M}_t$, observes the value of each pair in this matching, i.e. $Y_t = \{\f(\theta_u, \theta_v): (u, v)\in M_t^{\alg}\}$, and receives an instantaneous reward $\mu_{\f}(M_t^{\alg}) = \sum_{(u,v)\in M_t^{\alg}} \f(\theta_u, \theta_v)$. The set of permissible matchings has to satisfy the \emph{incremental matching constraint}: each $M\in \mathcal{M}_t$ is such that $M$ has at most two new matched pairs with respect to $M_{t-1}^{\alg}$. Formally, $\mathcal{M}_t = \{M\in \mathcal{M}: |M\Delta M_{t-1}^{\alg}| \leq 4\}$ where $\mathcal{M}$ is the set of all matchings, and $\Delta$ is the symmetric set difference operator $A\Delta B = \left(A \backslash B\right) \cup \left(B \backslash A\right)$. The algorithm $\alg$ specifies a mapping from the history  $\mathcal{H}_{t}$ to $M_t^{\alg}$, where $\mathcal{H}_1 = \emptyset$ and $\mathcal{H}_{t} = \{M_1^{\alg}, Y_1, \dots, M_{t-1}^{\alg}, Y_{t-1}\}$, for $t > 1$. See Figure~\ref{fig:inc-match} for an illustration.

An adaptive matching obeying the incremental matching constraint is referred to as an incremental matching algorithm. An adaptive incremental matching algorithm that in each round re-matches pairs of nodes greedily with respect to the conditional expected instantaneous regret in the next round according to the posterior belief about node states is referred to as a \emph{greedy Bayes algorithm}. For a given value function $\f$, we let $\gb$ denote a greedy Bayes algorithm. Note that we omit explicit referral to $\f$ in the notation $\gb$ for simplicity.

For any given value function $\f$, let $M^\ast$ be a maximum value matching of nodes in $V$, i.e. $M^\ast\in \arg\max_M \mu_w(M)$. Then, the \emph{regret} of an adaptive algorithm $\alg$ is defined as
$$
\breg_{\f}^{\alg}(T) = T \E[\mu_{\f}(M^\ast)] -  \E\left[\sum_{t=1}^T \mu_{\f}(M_t^{\alg})\right] 
$$
where in the right-hand side of the last equation, the expectations are taken with respect to the prior distribution of the node types and the prior distribution of node types and any randomization of algorithm $\alg$, respectively. Note that $\breg_{\f}^\alg(T)$ is the \emph{expected Bayesian regret}. We aim to characterise the asymptotic regret of greedy Bayes algorithm $\gb$ for some value functions $\f$ as the time horizon $T$ goes to infinity and the number of nodes $n$ goes to infinity. 

Note that for any value function $\f$ and any adaptive algorithm $\alg$, the initial matching is a random matching of nodes in $V$ because the prior distribution of node types is non-informative for maximum value matching. 

\subsection{Algorithms and regret bounds}
\label{sec:results}

We first show a regret lower bound that holds for any adaptive matching algorithm under mild assumptions. Let $\tilde{R}_{\f}$ denote the expected instantaneous regret incurred for a random matching of nodes and value function $\f$. The following lemma provides a regret lower bound that holds for any adaptive incremental matching algorithm. %\mv{*** More formal proof? ***}
%\jy{Updated}
%\jy{***translate it into a more general statement.***} \mv{*** Use the notation consistent with the rest of the paper, e.g. denoting the number of nodes with $n$ not $N$, referring to a pair value function not a pair testing function. ***} \mv{*** If the claim is a minor simple claim to establish, we may not want to present it as a theorem. ***}
%Here we show an asymptotic lower bound for any adaptive matching algorithm.

\begin{lemma}[lower bound]  For any adaptive incremental matching algorithm for value function $\f$, there exists a constant $c>0$ such that the expected regret is at least $c\tilde{R}_{\f}^2$, provided that $\tilde{R}_{\f}$ is larger than some constant value that depends only on $c$ and $\f$.
\label{lm:lb}
\end{lemma}

The proof of the lemma is provided in Appendix~\ref{lm:lb}. The proof follows by the fact that any adaptive incremental matching algorithm reduces the instantaneous regret in each round for at most a constant amount. From this and some simple arguments, it follows that the cumulative regret is lower bounded by the quadratic function of the expected instantaneous regret of initial random matching.

\begin{table}[t]
\caption{Regret lower bounds for different value functions.}
\begin{center}
\begin{tabular}{c | c}
$w$ & Regret lower bound\\\hline
OR & $\Omega(\min\{p,1-p\}^4 n^2)$\\
AND & $\Omega((p(1-p))^2 n^2)$\\
XOR & $\Omega(\min\{p,1-p\}^2 n^2)$\\
NXOR & $\Omega((p(1-p))^2 n^2)$\\
CES $0< a\leq 1$ & $\Omega((p(1-p))^2 n^2)$\\
CES $a > 1$ & $\Omega(\min\{p,1-p\}^4 n^2)$\\\hline
\end{tabular}
\end{center}
\label{tab:lb}
\end{table}

Regret lower bounds for different value functions are shown in Table~\ref{tab:lb}. These lower bounds follow from Lemma~\ref{lm:lb} and computations given in Appendix~\ref{sec:rnd}. For any fixed $0 < p < 1$, the regret lower bounds are $\Omega(n^2)$. All regret lower bounds scale as $\gamma^2 n^2$ when either $p = \gamma$ or $1-p=\gamma$ for some small $\gamma$, except for Boolean OR and CES $a > 1$ value functions in which case the regret lower bounds scale as $\gamma^4 n^2$. 

We will compare the regret upper bounds (which in some cases are tight) developed for greedy Bayes algorithms in the next sections and compare then with given lower bounds. Any additional factor in a regret upper bound that depends on the population parameter $p$ to the one that is present in the corresponding lower bound quantifies the search cost of a greedy Bayes strategy. 

We will see that different value functions $\f$ can be separated into two classes depending on whether or not they satisfy the constant improvement property. A value function is said to satisfy \emph{a constant improvement property} if in each round of the execution of the greedy Bayes algorithm, the instantaneous regret is guaranteed to be decreased for at least a constant amount $L$ over a constant number of next $M$ rounds, where $L$ and $M$ are constants that do not depend on either $n$ or $p$. For the class of value functions that satisfy the constant improvement property, the regret of a greedy Bayes algorithm is essentially determined by the instantaneous regret incurred in the initial random matching and the regret differs from the corresponding lower bound only for a constant factor. For value functions that do not satisfy the constant improvement property, the regret has an additional factor depending on the population parameter $p$ that is due to the search cost of the greedy Bayes algorithm. 


\subsubsection{Maximum value function (OR)}

In this section, we consider the maximum value function, defined as follows
$$
\f(x,y) = x \vee y.
$$

In this case, any optimal matching has the maximum number of matches of nodes of different types. Hence, an adaptive algorithm has to efficiently identify pairs of nodes of different types. Note that based on the observed value of a node pair, this node pair belongs to one of the following two sets $S_0 = \{(u, v): \f(\theta_u, \theta_v) = 0\}$ or $S_1 = \{(u, v): \f(\theta_u, \theta_v) = 1\}$. Here, $S_0$ is the set of all $0$-$0$ type pairs, and $S_1$ is the set of all $0$-$1$ and $1$-$1$ type pairs. Under the incremental matching constraint, the conditional expected reward is maximized by choosing one pair from $S_0$ and one pair from $S_1$ and rematching them. This strategy underlies the greedy Bayes algorithm. 

The main idea behind the algorithm is to exploit the \emph{known} low type nodes to explore the \emph{unknown} high type nodes. The algorithm maintains a set of node pairs known to be all of low type (thus each pair in this set has two nodes of low type) and a set of node pairs whose values were observed to be of high type (thus each pair in this set has at least one node of high type). In each round, the algorithm chooses a pair from the known set and a pair from the unknown set and then changes pairing of nodes of these two pairs. From observed pair values, the algorithm can identify the type of all nodes of the two chosen pairs. The algorithm terminates as soon as the types of all nodes in the unknown set are identified. The greedy Bayes algorithm corresponds to the 1-chain algorithm in \cite{KKL18}.

The asymptotic regret of the greedy Bayes algorithm is characterized in the following theorem.

\begin{theorem} \label{thm:max} For maximum value function $\f$, the regret of greedy Bayes algorithm satisfies
\begin{eqnarray*}
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) & \sim & \frac{1-(1-p)^2}{8p^2}\min\{p,1-p\}^4 n^2, \hbox{ for large } n.
\end{eqnarray*}
\end{theorem}

The proof of Theorem~\ref{thm:max} is provided in Appendix~\ref{app:max}. Here we provide the proof sketch. The key observation in the proof is that the instantaneous regret in each round is a linear function of the number of matches of $1$-$1$ type in the next round. We can show that the number of matches of $1$-$1$ type evolves according to a time-inhomogeneous Markov chain. The regret analysis boils down to computing the expected values of the states of this Markov chain until a stopping time at which either the number of matches known to be of $0$-$0$ type or the number of matches known to be either of $0$-$0$ or $0$-$1$ type is equal to zero. The analysis uses the Wormald's convergence theorem for bounding the expected value of some nonlinear functions of the Markov chain state. 

Under maximum value function, matching nodes of different type is preferred and the difficulty of finding the optimal matching is in removing all pairs of nodes of same type whenever possible. If the nodes are of predominantly of one type, i.e. when $p$ or $1-p$ is small, a minority-type node is matched with a node of the same type with a small probability in the initial random matching. This means that the initial random matching would typically be close to an optimal matching and, hence, the regret of the algorithm is small. In the other extreme, when there is a balanced number of nodes of different types, i.e. when $p$ is close to $1/2$, any node type is equally likely to be matched with a node of either type in the initial random matching. The initial random matching can thus be far from an optimal matching, and hence, the regret will be high. 

Theorem~\ref{thm:max} gives us a precise characterization of how the regret depends on the population parameter $p$. It indeed confirms the intuition that regret would be small when the population is predominantly of one type, and that the worst-case regret is achieved when there is a balanced number of node types. Observe that the dependency of the asymptotic regret on the population parameter $p$ is not symmetric around $1/2$. It can be readily checked that for any $0 < \gamma < 1/2$, the asymptotic regret when $p = \gamma$ is larger than the asymptotic regret when $p = 1-\gamma$. In the limit of small $p$, the asymptotic regret is approximately $(1/4) p^3 n^2$, while in the limit of small $1-p$, the asymptotic regret is approximately $(1/8)(1-p)^4 n^2$. This shows tƒhat it is harder to find an optimal matching by greedy search when $p$ is small (many low-type nodes) than when $1-p$ is small (many high-type nodes). 

Compared with the lower bound shown in Table~\ref{tab:lb}, the regret upper bound has the extra factor $(1-(1-p)^2)/p^2 = (2-p)/p$. This extra factor quantifies the regret due to the search cost of the greedy Bayes algorithm. This extra factor scales as $1/p$ for small value of $p$. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=7cm]{regret-max.png}
\caption{The asymptotic normalized regret for maximum value function, in the limit of large number of nodes $n$, versus population parameter $p$.}
\label{fig:regret-max}
\end{center}
\end{figure}


\subsubsection{Minimum value function (AND)} \label{sec::and}

In this section we consider the case of minimum value function defined as
$$
\f(x,y) = x\wedge y.
$$
Under minimum value function, a greedy Bayes algorithm aims at searching for high-type nodes in order to match them together, as only in this case a positive reward is accrued.

The posterior distribution of node types can be represented by a collection of sets, each of which we refer to as a  \emph{matching set}, and the identities of nodes whose types are determined with certainty from observed pair values. Each matching set contains a set of matches such that there is \emph{at most one node} of high type in this set. The greedy Bayes algorithm explores pairs of nodes that reside in different matching sets, and, as we will show, prioritizes the search to matching sets of smallest size.

For any two matching sets, evaluation of all pairs of nodes belonging to these two matching sets results in two possible outcomes: either (a) a $1$-$1$ match is found, in which case the two matching sets are removed from further consideration, or (b) a $1$-$1$ match is not found, in which case the two matching sets are merged into a new matching set. In the former case, each matching set has exactly one high-type node, and having found a match between the two high-type nodes, all other nodes in the two matching sets are identified to be of low-type with certainty. On the other hand, in the latter case, having not found a $1$-$1$ match of nodes spanning the two matching sets, the only information deduced from observed pair evaluations is that there is at most one high-type node in the union of the two matching sets. Hence, in this case we merge the two matching sets into a new matching set. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{merge-and.pdf}
\caption{An illustration of evolution of matching sets of greedy Bayes matching strategy for AND value function.}
\label{fig:and-merge}
\end{center}
\end{figure}


This exploration procedure ends when matching sets coalesce into one set or no matching set remains. In the former case, the remaining matching set contains at most one high-type node, which cannot be matched with any other high-type node as all of them are already matched to a high-type node. 

The following is a key lemma to show that greedy Bayes strategy explores matching sets of smallest sizes first. 

\begin{lemma} For every round of greedy Bayes algorithm and every set of matches $A$ of cardinality $a$ for which the available information is that $A$ contains at most one high-type node, the posterior probability of $A$ containing a high-type node is 
$$
\pp(a) = \frac{pa}{1-p+pa}.
$$ 
\label{lm:pa}
\end{lemma}

The proof of the lemma is provided in Appendix~\ref{sec:pa}. The proof is by induction over cardinality of matching sets. 

Note that the posterior probability of a matching set containing a high-type node depends only on its cardinality. Intuitively, the larger the cardinality of a matching set, the larger the posterior probability of this matching set containing a high-type node. Note that any specific node in a matching set $A$ of cardinality $a$ is a high-type node with probability $\pp(a)/(2a) = p/(2(1-p+pa))$, which is decreasing in the cardinality of $A$. This implies that the greedy Bayes strategy is to explore pairs of nodes residing in two different matching sets of smallest size. 

We refer to greedy Bayes algorithm for minimum value function as {\sc Least-Size-Merge} algorithm, which is formally defined in Algorithm~\ref{alg:min}. This algorithm uses a procedure {\sc Is-Merge} defined in Algorithm~\ref{alg::ismerge}. This procedure uses as input two matching sets and constructs matchings of nodes by exploring pairs of nodes residing in the two matching sets.   

\begin{algorithm}[ht]
\caption{Least-Size-Merge}
\label{alg:min}
\SetKwInOut{Init}{Initialization}
\SetKwInOut{Input}{Input}
\Input{nodes set $N$.} 
\Init{iteration $t=1$, $M_1\gets$ a random matching on nodes $N$ and $S\leftarrow \{\{(i, j)\}\in M_1 : Y_1(i,j)= 0\}$.}
\While{$|S| > 1$}{
    $A \leftarrow \underset{S'\in S}{\arg\min} |S'|$\;
    $B \leftarrow \underset{S'\in S\backslash \{A\}}{\arg\min} |S'|$\;
    $S \leftarrow S \backslash \{A, B\}$\;
    \If{IS-MERGE$(A, B) ==$ True}{
        $S \leftarrow S \cup \{A \cup B\}$
    }
}
\end{algorithm}

From the above discussion, it is clear that greedy Bayes algorithm results in a stochastic process that describes evolution of a collection of matching sets as pairs of matching sets are examined, which results in either merging two matching sets or removing them from the collection of matching sets.  

The initial matching is a random matching. From this initial matching, the algorithm identifies high-type nodes that belong to matches yielding value $1$, and a set of matching sets, each consisting of a pair of nodes for which the evaluation is observed to be of value $0$. Indeed, all pairs in these matching sets are either of $0$-$0$ or $0$-$1$ type. Let $X_1$ be the number of matching sets at step $1$. It is readily observed that
$$
X_1 \sim \mathrm{Bin}\left(\frac{n}{2}, 1-p^2\right).
$$

We divide rounds into epochs. In each epoch $r$, let $S_r$ denote the set of matching sets at the beginning of epoch $r$. Initially, as we discussed, $S_1$ consists of pairs of type $0$-$0$ or $0$-$1$ defined by the initial random matching and the cardinality of this set is $X_1$. At epoch $r$, a pair of matching sets $A$ and $B$ of the smallest size is removed from $S_r$ and pairs of nodes spanning $A$ and $B$ are evaluated until either a match $1$-$1$ is found, or not such a match is found. In the latter case, we deduce that nodes in $A\cup B$ contain at most one high-type node. The set of matching sets in the next epoch,  $S_{r+1}$, consists of all unexplored matching sets from $S_r$, and $A\cup B$ if the outcome of examining $A$ and $B$ resulted in not finding a $1$-$1$ match.

In each epoch, the posterior distribution of node types is fully defined by the identities of nodes inferred to be of high-type, and the set of matching sets. The posterior probability of a matching set containing a high-type node is given in Lemma~\ref{lm:pa}. 

\begin{algorithm}[ht]
\caption{IS-MERGE}
\label{alg::ismerge}
\SetKwInOut{Init}{Initialization}
\SetKwInOut{Input}{Input}
\Input{two matching sets $A, B$.}
\Init{create a candidate set $P_i \leftarrow B$ for all $i\in A$}
\For{all node $u\in A$}{
    \While{$P_u \neq \emptyset$}{
    $t\leftarrow t+1$\;
    choose an node $v\in P_u$ and let $(u, u'), (v, v') \in M_{t-1}$\;
    $M_t\gets (M_{t-1}\backslash\{(u, u'), (v, v')\} \cup \{(u, v), (u', v')\}$\;
    \If{$Y_t(u, v) + Y_t (u', v') = 1$}{
        \textbf{return} False\;
    }
    $P_{u} \leftarrow P_{u} \backslash \{v\}$\;
    \If{$u'\in A$}{
        $P_{u'} \leftarrow P_{u'} \backslash \{v'\}$\;
    }
    \If{$v'\in A$}{
        $P_{v'} \leftarrow P_{v'} \backslash \{u'\}$
    }
    }
    \textbf{return} True\;
}

\end{algorithm}

It is readily observed that at the beginning of each epoch, all matching sets are of the same cardinality except for at most one set of larger cardinality. We call this latter matching set a \emph{special matching set}, if one exists, and all other as \emph{regular matching sets}.

As the greedy strategy prioritizes evaluating nodes residing in smallest matching sets, we can divide epochs in super-epochs. In each super-epoch, disjoint pairs of regular matching sets are created and are then examined in arbitrary order, and if there is a special matching set, it is paired at the end of the super-epoch with a regular set for examination. For super-epoch $s$, let $X_s$ denote the number of regular matching sets and let $Y_s$ denote the cardinality of the special matching set; if there is no special matching set, we define $Y_s = 0$. 

Stochastic process $\{(X_s, Y_s)\}_{s\geq 0}$ is a Markov chain with initial state$(X_0,Y_0) = (n/2, 0)$, and for each super-epoch $s\geq 0$, 
\begin{equation}
X_{s+1} \mid (X_s,Y_s) \sim \mathrm{Bin}\left(\left\lfloor\frac{X_s}{2}\right\rfloor, 1-\pp(2^s)^2\right)
\label{equ:X}
\end{equation}
and
\begin{equation}
Y_{s+1} \mid (X_s,Y_s,X_{s+1}) \sim 
\left\{\begin{array}{ll}
(Y_s+\xi_s)\mathrm{Ber}\left(1-\pp(\xi_s)\pp(Y_s)\right) & \hbox{ if } Y_s > 0\\
(2^s + 2^{s+1})\mathrm{Ber}\left(1-\pp(2^s)\pp(2^{s+1})\right) & \hbox{ if } Y_s = 0, X_s \hbox{ is odd}, X_{s+1}>0\\
0, & \hbox{ otherwise}
\end{array}\right .
\label{equ:Y}
\end{equation} 
where 
$$
\xi_s = \left\{
\begin{array}{ll}
2^s & \hbox{ if } X_s \hbox{ is odd}\\
2^{s+1} & \hbox{ if } X_s \hbox{ is even, and } X_{s+1} > 0\\
0 & \hbox{ otherwise}
\end{array}
\right . .
$$
%and, if $Y_s = 0$, $X_s$ is odd, and $X_{s+1} > 0$,
%$$
%Y_{s+1} \mid (X_s,Y_s) \sim (2^s + 2^{s-1})\mathrm{Ber}\left(1-p(2^s)p(2^{s+1})\right)
%$$
%and, otherwise, $Y_{s+1} \mid (X_s, Y_s) = 0$.

The transition probabilities of the Markov chain $\{(X_s,Y_s\}_{s\geq 0}$ can be interpreted as follows. In each super-epoch, matchings are first created by swapping matches for nodes belonging to different regular matchings sets, by examining one pair of regular matching sets after other. There are $\lfloor X_s/2\rfloor$ pairs of regular matching sets that are examined in super-epoch $s$. Each such examination of a pair of regular matching sets $A$ and $B$ results in either $A$ and $B$ being merged, which occurs with probability $1-\pp(|A|)\pp(|B|)$, or $A$ and $B$ being removed from further consideration which occurs with probability $\pp(|A|)\pp(|B|)$.  Observe that $\pi(|A|)\pi(|B|)$ is the probability that both $A$ and $B$ contain a high-type node. The outcomes of this procedure are illustrated in Figure~\ref{fig:merge}. All regular matching sets in super-epoch $s$ are of cardinality $2^s$. Hence, in super-epoch $s$, two regular matching sets are merged with probability $1-\pp(2^s)^2$, and are removed from further consideration with probability $\pp(2^s)^2$. This explains the conditional distribution of the number of regular matching sets in super-epoch $s+1$, $X_{s+1}$, given in (\ref{equ:X}). 

\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.7\linewidth]{merge.pdf}
\caption{Two possible outcomes: merge or remove two matching sets.}
\label{fig:merge}
\end{center}
\end{figure*}

We next explain the conditional distribution of the cardinality of the special set in super-epoch $s+1$, $Y_{s+1}$, conditional on the values of $X_s, Y_s$ and $X_{s+1}$ given by (\ref{equ:Y}). There are three possible cases. First, if $Y_s > 0$, then at the beginning of super-epoch $s$ there is a special matching set of cardinality $Y_s$. This set is examined with a matching set $A$ of cardinality $\xi_s$ at the end of super-epoch $s$ after regular matching sets are examined, if there is at least one matching set left for consideration besides the special matching set. The set $A$ is either (a) one of regular matching sets of cardinality $2^{s}$ if at the beginning of super-epoch $s$ the number of regular matching sets is odd, or (b) a matching set of cardinality $2^{s+1}$ that resulted from merging two regular matching sets in super-epoch $s$ if the number of regular matching sets at the beginning of super-epoch $s$ is even and at least one merging resulted from examinations of regular matching sets. Second, if $Y_{s}=0$, then all matching sets at the beginning of super-epoch $s$ are regular matching sets. In this case, a special matching set can exist in super-epoch $s+1$, only if the number of regular matching sets at the beginning of super-epoch $s$ is odd and at least one merging resulted from examination of regular matching sets in super-epoch $s$. The cardinality $Y_{s+1}$ of this special set is clearly $2^s+2^{s+1}$. Finally, if $Y_s = 0$ and either number of regular matching sets at the beginning of super-epoch $s$ is even or no examination of regular matching sets in super-epoch $s$ resulted in merging, there is no special matching set in super-epoch $s+1$. Note that cardinality of the special matching set in super-epoch $s$ is of cardinality $Y_1=0$ for $s = 1$ and $Y_s \leq 2^1 + \cdots + 2^s \leq 2^{s+1}$ for $s > 1$. 

The Markov chain $\{(X_s, Y_s)\}_{s\geq 0}$ has absorbing states $(0,0)$, $(1,0)$, $(0,z)$, for $0<z\leq n$. In state $(0,0)$, all high-type nodes are identified. In states $(1,0)$ or $(0,z)$, there is at most one unidentified high-type node. It is not needed to identify the type of this node, as all other high-type nodes are already matched with high-type nodes. 

The number of rounds for examination of a pair of matching sets is discussed as follows. For any two matching sets $A$ and $B$, with cardinalities $|A|=a$ and $|B| = b$, let $N(a,b)$ be the smallest number of adjacent matchings that cover all pairs $(u,v) \in A\times B$. It can be readily noted that $ab/2\leq N(a,b)\leq ab$. When exploring pairs in matching sets $A$ and $B$ such that either $A$ or $B$ contains only low-type nodes, the number of exploration steps is equal to $N(a,b)$. On the other hand, when exploring pairs in matching sets $A$ and $B$ such that both $A$ and $B$ contain a high-type node, then the number of exploration steps is a random variable with expected value $N(a,b)/2$.

The number of steps until {\sc Least-Size-Merge} algorithm terminates is characterised in the following proposition.

\begin{proposition} The expected number of steps $\tau$ until termination of algorithm {\sc Least-Size-Merge} is bounded as follows
$$
\E[\tau] = O\left(\min\left\{\frac{n}{p},n^2\right\}\right).
$$
\label{pro:epochs}
\end{proposition}



\begin{figure*}[t]
\begin{center}
$n = 128$ \hspace*{5.5cm} $n = 256$\\
\includegraphics[width=7cm]{min-ite-n128.png}
\includegraphics[width=7cm]{min-ite-n256.png}\\
$n = 512$ \hspace*{5.5cm} $n = 1024$\\
\includegraphics[width=7cm]{min-ite-n512.png}
\includegraphics[width=7cm]{min-ite-n1024.png}
%\includegraphics[width=0.24\linewidth]{min-itelog-n128.png}
%\includegraphics[width=0.24\linewidth]{min-itelog-n256.png}
%\includegraphics[width=0.24\linewidth]{min-itelog-n512.png}
%\includegraphics[width=0.24\linewidth]{min-itelog-n512.png}
\caption{The number of rounds until greedy Bayes incremental matching algorithm terminates for minimum (Boolean AND) value function versus population parameter $p$, for different numbers of nodes $n$. %from left to right $n = 128,256,512,1024$. 
%\mv{*** Run the new code to obtain the plots to update the plots ***)}
}
\label{fig:min-ite}
\end{center}
\end{figure*}

%The length of the super-epoch $s$, denoted as $T_s$, can be expressed as follows. 
%\begin{eqnarray*}
%T_s &=& N(2^s,2^s)X_{s+1} + \sum_{i=1}^{\left\lfloor \frac{X_s}{2}\right\rfloor - X_{s+1}} N_i \\
%&& + N(\xi_s, Y_s)\ind_{\{Y_{s+1} > 0\}}\\x
%&& + N_0 \ind_{\{Y_{s+1} = 0\}}
%\end{eqnarray*}
%where $N_i$ are independent and identically distributed random variables with distribution $N_i \sim \mathrm{Bin}(N(2^s,2^s),1/2)$, and $N_0\sim \mathrm{Bin}(N(\xi_s,Y_s),1/2)$ conditional on $\xi_s$ and $Y_s$. 

%\mv{*** Check the proof whether we use any assumptions on $p$, e.g. $p$ being a fixed constant, and then letting $n$ grow. Also for our other theorems. ***}
%\jy{checked. this holds as long as $p\leq 1$.}

\begin{theorem} \label{thm:min-reg}
For minimum value function $\f$, the regret of greedy Bayes algorithm {\sc Least-Size-Merge} satisfies
$$
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) \leq \left( a_{n, p} + b_{n,p}\right) n^2 + O(n^2\log(n)), \hbox{ for large } n
$$
where
$$
a_{n, p}=\frac{1}{4} \sum_{s=1}^{\log _{2}(n)} \left(1- \frac{1}{2}p_s\right) \left(1-\frac{1}{2}p_s^2\right) p_s\left(\prod_{i=0}^{s-1} q_{i}^{2}+\frac{1}{n} \sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=0}^{i} q_{j}\right)\left(\prod_{j=i+1}^{s-1} q_{j}^{2}\right)\right),
$$
$$
b_{n,p}= \frac{1}{n} \sum_{s=1}^{\log _{2}(n)}  2^{s+1}  p_{s}\left(1-p_{s}\right) \prod_{i=0}^{s-1} q_{i}
$$
with $p_s = p2^s/\left(1-p+p2^s\right)$ and $q_s = 1 - p_s^2$. 

The sequences $a_{n,p}$ and $b_{n,p}$ have the following properties:
\begin{enumerate}
\item[(i)] $a_{n, p}=b_{n,p}=0$ for $p=0$ and $p=1$, for all $n$.
\item[(ii)] $a_{n,p} \leq c$ and $b_{n,p}\leq c$ for all $n$ and $p$, for some universal constant $c$.
\item[(iii)] For $1/2 < p \leq 1$, 
$$
a_{n,p} \leq \left(\left(\frac{1-p}{p}\right)^2 + \left(\frac{1-p}{p}\right)^4 + \frac{1}{4}\left(1+\frac{1}{3\cdot 2^{5/4}\log(2)}\right)\left(\frac{1-p}{p}\right)^{6}\right)\left(1+O\left(\frac{\log(n)}{n}\right)\right)
$$
and $$
b_{n,p} \leq O\left(\left(1-p\right)^2\frac{1}{n}\right).
$$
\item[(iv)] For $p\leq c/n$ for an arbitrarily fixed constant $c$, 
$$
a_{n,p} \leq \frac{1}{4}\log_2\left(\frac{1}{\sqrt{c}}\right) + \frac{3}{4}\frac{1}{1-c} + o(1)
$$
and 
$$
b_{n,p} = \frac{1}{2}\frac{1}{1-c} + o(1).
$$
\end{enumerate}

\label{thm:min}
\end{theorem}

Proof of the theorem is provided in Appendix~\ref{thm:min-reg}. The proof separately considers contributions to regret over rounds at which regular matching sets are examined and contributions to regret over rounds at which a special set is examined. 

In the regret bound, $a_{n,p}$ is due to regret accumulated while examining regular matching sets while $b_{n,p}$ is due to regret accumulated while examining a special matching set. Property (i) is intuitive as when $p = 0$ or $p = 1$ then any algorithm has a zero regret. Property (ii) tells us that regret is $O(n^2)$ for any scaling of $p$ with $n$. Property (iii) gives us an explicit regret bound and implies that regret is bounded by $(1-p)^2 n^2 + O(n)$ asymptotically for large $n$ and small $1-p$. Property (iv) gives an explicit regret bound when $p\leq c/n$ for some constant $c$.



In Figure~\ref{fig:min-reg}, we show the theoretical regret bound in Theorem~\ref{thm:min} along with the regret estimated through simulations versus the value of population parameter $p$ for several different values of the number of nodes $n$. We observe that the theoretical bound is tight for large values of $n$. Observe that the regret decreases with the value of the population parameter $p$ for any sufficiently large value of this parameter. This is intuitive as for pair values according to the MIN function, the goal is to maximize the number of $1$-$1$ type matches, which  easier for greedy search when there is a larger number of high-type nodes.

%We consider an arbitrary super-epoch $s$. Condition on $\tilde{X}_s$ and $\tilde{Y}_s$ where $\tilde{X}_s$ is the number of type-$1$ nodes in $X_s$ normal sets of size $2^s$ and $\tilde{Y}_s = 1$ if the special set, if there exists one, contains a type-$1$ item, and $\tilde{Y}_s = 0$, otherwise. For simplicity of notation, we write $\tilde{x}$, $x$, $\tilde{y}$ and $y$ in lieu of $\tilde{X}_s$, $X_s$, $\tilde{Y}_s$, and $Y_s$, respectively.

%The instantaneous regret at the beginning of super-epoch $s$ is given as follows. If $\tilde{x}$ is even, then the instantaneous regret is $\tilde{x}/2$. If $\tilde{x}$ is odd, then the instantaneous regret is $(\tilde{x}-1)/2$ if $\tilde{y} = 0$ and $(\tilde{x}+1)/2$ if $\tilde{y} = 1$. Hence, the initial instantaneous regret is
%$$
%R_0 = \left\lfloor \frac{\tilde{x}}{2}\right\rfloor + \tilde{y} \ind_{\{\tilde{x} \hbox{ odd }\}}.
%$$

%We next consider the regret over epochs in super-epoch $s$. We can think of each epoch as drawing two sets without replacement from an initial set containing $X_s$ sets of nodes. Let $K_r$ be the number of draws of a pair of sets each containing a type-$1$ item. Let $L_r$ be the number of draws of a pair of sets such that one of them contains only type-$0$ nodes and other contains a type-$1$ node by epoch $r$. Note that $r - K_r - L_r$ is the number of draws of a pair of sets, each containing only type-$0$ nodes. 

%Note that $\{(K_r, L_r)\}_{r\geq 0}$ is a Markov chain with transition probabilities defined by
%$$
%\left(
%\begin{array}{c} K_{r+1}\\ L_{r+1}\end{array}
%\right) = 
%\left(
%\begin{array}{c} K_{r}\\ L_{r}\end{array}
%\right)
%+ \left(
%\begin{array}{c} 0\\ 1\end{array}
%\right) \xi^{01}_r
%+
%\left(
%\begin{array}{c} 1\\ 0\end{array}
%\right) \xi^{11}_r
%$$
%where $(\xi^{01}_r,\xi^{11}_r)$ are random variables with conditional distribution 
%$$
%\P[(\xi^{01}_r, \xi^{11}_r)=(a,b)\mid K_r =k, L_r = l] = %p_{ab}(r,k,l)
%$$ 
%with
%\begin{eqnarray*}
%p_{01}(r,k,l) &=& 2\frac{x-\tilde{x}-l}{x-2r}\frac{\tilde{x}-2k-l}{x-2r-1}\\
%p_{11}(r,k,l) &=& \frac{\tilde{x}-2k-l}{x-2r}\frac{\tilde{x}-2k-l-1}{x-2r-1}\\
%p_{00}(r,k,l) &=& 1-p_{01}(r,k,l) - p_{11}(r,k,l).
%\end{eqnarray*}

%The instantaneous regret is decremented by $1$ in each epoch in which the draw is a pair of sets both containing a type-$1$ item. Hence, we have
%$$
%R_{r+1} = R_r - \xi_r^{11}.
%$$

%The expected cumulative regret $A_r$ by epoch $r$ evolves, starting from initial value $A_0 = 0$, according to, for $r \geq 0$,
%$$
%A_{r+1} = A_r + R_r (\alpha (1-\xi^{11}_r) + \beta \xi^{11}_r) 
%$$
%where $\alpha$ is the expected number of steps of an epoch in which the draw is a pair of sets with at least one of them containing only type-$0$ nodes and $\beta$ is the expected number of steps of an epoch in which the draw is a pair of sets both containing a type-$1$ item. 

%The expected cumulative regret in the super-epoch at the time when all pairs of normal sets are explored is equal to $\E[A_{\lfloor x/2 \rfloor}]$. In the given super-epoch, there may be an additional regret incurred during exploration of pairs between the special set and a normal set. This can occur only if $x$ is odd, and there is a special set. The instantaneous regret is equal to
%$$
%Q := \left\lfloor\frac{\tilde{x}-2K_{[x/2]} + \tilde{y}}{2}\right\rfloor.
%$$
%Note that the normal set with which the special set is paired contains only type-$0$ nodes if $\tilde{x} - (2K_{[x/2]}-L_{[x/2]}) = 0$, and otherwise contains a type-$1$ node if $\tilde{x} - (2K_{[x/2]}-L_{[x/2]})=1$. Let 
%$$
%E : = \{\tilde{x} - (2K_{[x/2]}-L_{[x/2]}) = 0\}. 
%$$
%The number of time steps of the last epoch can be expressed as follows
%$$
%T = N(2^s, y)\ind_{\{E\}} + \tilde{N}(2^s, y) \ind_{\{E^c, \tilde{y}=1\}} 
%$$
%where $\tilde{N}(2^s,y)$ is the number of steps it takes to discover a $1$-$1$ match. 

%The total regret incurred in the last epoch is equal to $Q T$.



\begin{figure*}[t]
\begin{center}
% \includegraphics[width=0.24\linewidth]{min-reg-n128.png}
% \includegraphics[width=0.24\linewidth]{min-reg-n256.png}
% \includegraphics[width=0.24\linewidth]{min-reg-n512.png}
% \includegraphics[width=0.24\linewidth]{min-reg-n1024.png}
$n = 1024$ \hspace*{5.5cm} $n = 2048$\\
\includegraphics[width=7cm]{min-bound-n1024.png}
\includegraphics[width=7cm]{min-bound-n2048.png}\\
$n = 4096$ \hspace*{5.5cm} $n = 8192$\\
\includegraphics[width=7cm]{min-bound-n4096.png}
\includegraphics[width=7cm]{min-bound-n8192.png}
\caption{Regret of the greedy Bayes algorithm for the MIN value function versus the population parameter $p$, for different values of the number of nodes $n$.}
\label{fig:min-reg}
\end{center}
\end{figure*}


\subsubsection{Affinity value function (NXOR)}

In this section we consider the affinity value function defined as follows
$$
\f(x,y) = x\wedge y + (1-x)\wedge (1-y).
$$
We refer to this function as the affinity value function because it outputs value $1$ for every pair of nodes of the same type, and otherwise outputs value $0$. Such a value function is of interest, for example, in online gaming and other competitions where the the goal is to match players of similar skills, and in social networks where higher value arises from social interactions between users of similar interests---the value function measuring affinity between two users.

Having evaluated values of node pairs for any given matching $M$ of nodes, the algorithm can identify pairs of nodes of different types ($0$-$1$ type pairs) with certainty. The greedy Bayes strategy amounts to re-matching nodes belonging to pairs of nodes known to be of $0$-$1$ type. 

\begin{theorem} For affinity value function $\f$, the regret of greedy Bayes algorithm satisfies
$$
\lim_{T\rightarrow \infty} R_{\f}^\gb(T) \sim \frac{3}{8}(p(1-p))^2 n^2, \hbox{ for large } n.
$$
\label{thm:aff}
\end{theorem}

Proof is provided in Appendix~\ref{sec:aff}. The proof is rather simple as the dynamics is simple -- it amounts to sequential examinations of pairs of node pairs known to be of $0$-$1$ type. The affinity value function clearly satisfies the constant improvement property, thus the regret upper bound matches the lower bound in Table~\ref{tab:lb} up to a constant factor. The regret achieves the highest value for $p = 1/2$ and decays in a symmetric way with the distance between $p$ and $1/2$.

\subsubsection{Dissimilarity value function (XOR)}

We consider the dissimilarity value function, which corresponds to the Boolean XOR function, defined as follows 
$$
\f(x, y) = x (1-y) + (1-x)y
$$
This value function outputs $1$ for any pair of nodes of different types, and, otherwise, outputs value $0$ -- hence the name, dissimilarity function. 

The maximum reward is achieved by a matching that has the highest number of matches of nodes of different types. Hence, for any set of nodes with $N_1$ nodes of value $1$, the maximum weight matching has value
$$
\mu^\ast = \min \{n - N_1, N_1\}.
$$
For each time step $t$, let $U_t$ and $K_t$ denote the number of matches of nodes of the same and different type, respectively, and let $V_1$ denote the number of matches of $1$-$1$ type nodes. Then, note that $U_t + K_t = n/2$ and $N_t = 2V_t+K_t$ for all $t\geq 1$, and the instantaneous regret can be expressed as follows
$$
R_t =\mu^\ast - K_t =  U_t - \left|U_1-2V_1\right|.
$$

Suppose that we have two pairs of nodes, with each pair of value $0$, i.e. each pair consists of nodes of the same type. By re-matching each node from one pair to a node in the other pair, and observing values of newly formed pairs, we have two possible outcomes (a) each of the two new pairs consists of nodes of different types, hence each pair having value $1$, or (b) we conclude that all four nodes are of the same type. 
Similarly as in Section~\ref{sec::and}, we call a set of node pairs a matching set when we know with certainty that all pairs in this set consists of nodes of same type. 
The following lemmas show that the greedy Bayes strategy is to keep re-matching nodes belonging to matching sets of smallest size.

\begin{lemma} 
For every round of greedy Bayes algorithm and any matching set of $a$ matches, the posterior probability that a randomly sampled node pair from this matching set is of type $1$-$1$ is 
$$
\pi(a) = \frac{p^{2a}}{p^{2a} + (1-p)^{2a}}.
$$
\label{lm:alpha-function}
\end{lemma} 

Proof is provided in Appendix~\ref{sec:alpha-function}. The proof is based on induction over cardinality of matching sets. 

\begin{lemma}
For any collection of two or more matching sets, the expected reward is largest for re-matching two matches uniformly sampled from two matching sets of smallest size.
\label{lm:xor-gb}
\end{lemma}

The proof of the lemma is provided in Appendix~\ref{sec:xor-gb}. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{xor-merge.pdf}
\caption{An illustration of evolution of matching sets of greedy Bayes matching strategy for XOR value function.}
\label{fig:xor-merge}
\end{center}
\end{figure}


The greedy Bayes adaptive matching algorithm is defined in Algorithm~\ref{alg:xor}. Similarly to  Algorithm~\ref{alg:min}, a set of matching sets is maintained and the number of matching sets is non-increasing in every round of the algorithm.
The algorithm stops when there is only one matching set left, if any. See Figure~\ref{fig:xor-merge} for an illustration.
In each round, two matching sets of  smallest sizes are selected to perform the {\sc Merge-Xor} operation and the output of this operation is added to the set of matching sets.
In the {\sc Merge-Xor} operation, a matched pair of nodes is selected from each input matching set randomly and the two selected node pairs are re-matched. 
When the two re-matched pairs are observed to be of value $1$, the nodes in the two matching sets are of different types.
Otherwise, the two matching sets have the same type of nodes and hence are merged into one matching set which is added to the set of matching sets.

\begin{algorithm}[ht]
\caption{Least-Size-Merge-XOR}
\label{alg:xor}
\SetKwInOut{Init}{Initialization}
\SetKwInOut{Input}{Input}
\Input{nodes set $N$.} 
\Init{iteration $t=1$, $M_1\gets$ a random matching on nodes $N$ and $S\leftarrow \{\{(i, j)\}\in M_1 : Y_1(i,j)= 0\}$.}
\While{$|S| > 1$}{
    $A \leftarrow \underset{S'\in S}{\arg\min} |S'|$\;
    $B \leftarrow \underset{S'\in S\backslash \{A\}}{\arg\min} |S'|$\;
    $S \leftarrow S \backslash \{A, B\}$\;
    $S \leftarrow S \cup $ MERGE-XOR($A, B$)\;
}
\end{algorithm}


\begin{algorithm}[t]
    \caption{MERGE-XOR}
    \label{alg::merge-xor}
    \SetKwInOut{Init}{Initialization}
    \SetKwInOut{Input}{Input}
    \Input{two matching sets $A, B$.} 
            \While{$A\neq\emptyset$ and $B\neq\emptyset$}{
                uniformly sample two pairs: $(u_A, v_A)\in A$ and $(u_B, v_B)\in B$\;
                $t\to t+1$\;
                \If{$(u_A, u_B) = 0$}{
                    \textbf{return} $\{A\cup B\}$\;
                }
                \Else{
                    $t\to t+1$\;
                    $K \to K \cup \{(u_A, u_B), (v_A, v_B)\}$\;
                }
            }
           \textbf{return} $\{A\cup B\}$\;
\end{algorithm}

\begin{figure*}[ht]
\begin{center}
$n = 1024$ \hspace*{5.5cm} $n = 2048$\\
\includegraphics[width=7cm]{xor-bound-n1024.png}
\includegraphics[width=7cm]{xor-bound-n2048.png}\\
$n = 4096$ \hspace*{5.5cm} $n = 8192$\\
\includegraphics[width=7cm]{xor-bound-n4096.png}
\includegraphics[width=7cm]{xor-bound-n8192.png}
\caption{Regret of the greedy Bayes algorithm for the XOR value function versus the population parameter $p$, for different values of the number of nodes $n$.}
\label{fig:xor-reg}
\end{center}
\end{figure*}

\subsubsection{CES value function}

We consider the constant elasticity of supply (CES) function defined as as follows, for parameter $a>1$,
$$
\f(x,y) = (x^a + y^a)^{1/a}.
$$
This function is commonly studied as a production function in economic literature, where $0 < a \leq 1$ is referred to as the substitutes case and $a>1$ as the complements case. In our case, individual inputs are Boolean, hence the function outputs $0$ for for a pair of nodes of low type, $1$ for a pair of nodes of different types, and $2^{1/a}$ for a pair of nodes of high type. Note that for Boolean inputs the function is alike to maximum value function (Boolean OR), except for returning a value larger than $1$ for $(0,0)$ input. For the CES value function, there is an ambiguity about individual node types, upon testing a pair of nodes, only if the two nodes are of different types. The regret of greedy Bayes matching is different for the case of substitutes and complements. 

\paragraph{Substitutes case $0 < a \leq 1$}

The total value of any two node pairs of $0$-$1$ type is equal to $2$, while the total value of two node pairs of $0$-$0$ and $1$-$1$ type is equal to $2^{1/a}$. Under assumption $0 < a\leq 1$, it holds $2^{1/a} \geq 2$ where the equality holds only in the case when $a = 1$. It follows that when $0< a < 1$, it is always beneficial to rematch two pairs of $0$-$1$ type to create two pairs of $0$-$0$ and $0$-$1$ type. 

The following lemma gives a necessary and sufficient condition for a matching to be optimal.

\begin{lemma} For value function $\f$ being the CES function with $0 < a < 1$, a matching is optimal if, and only if, it contains at most one pair of nodes of different types. Otherwise, if $a = 1$, then any matching is an optimal matching. 
\label{lm:cesop1}
\end{lemma}

%\mv{*** Why Lemmas 4.1 and 4.2 give different properties of optimal matchings? - while the same amount of information is extracted from each pair test, and only the reward is affected. ***}

The above discussion and Lemma~\ref{lm:cesop1} tell us that a greedy Bayes algorithm prioritizes creating $1$-$1$ pairs by rematching pairs of $0$-$1$ type. Note that the algorithm can identify all there pair types, namely $0$-$1$, $0$-$0$ and $1$-$1$, from observed pair values. In each round, the greedy Bayes algorithm selects two $0$-$1$ type pairs and rematches them until finding two pairs of $1$-$1$ and $0$-$0$ type, with all other pairs remaining the same.
The algorithm terminates when there is at most one pair of $0$-$1$ type in the matching. Note that in each round the greedy Bayes algorithm is guaranteed to decrease the regret for at least $2^{1/a}-2$ over the next two rounds. Hence, the CES $0 < a \leq 1$ function satisfies the constant improvement property. 
%\mv{*** TBD - the algorithm needs to be defined more clearly. ***} \jy{updated.}
 
\begin{theorem} For CES value function $\f$ with $0 < a \leq 1$, the regret of greedy Bayes algorithm satisfies
$$
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) \sim \frac{3}{4}(2^{1/a}-2)(p(1-p))^2 n^2, \hbox{ for large } n.
$$
\label{thm:ces1}
\end{theorem}

Proof of Theorem~\ref{thm:ces1} is provided in Appendix~\ref{app:ces1}. The proof is simple because the underlying dynamics is simple. The algorithm examines two pairs of $0$-$1$ type one after other, and re-matches nodes of these two pairs until two pairs of $1$-$1$ and $0$-$0$ type are found. Each such examination takes either one or two steps. The number of examinations is equal to the number of pairs of matches of $0$-$1$ type in the initial random matching. The regret analysis boils down to accounting for expected regret accrued in each examination of two pairs of $0$-$1$ type.

The asymptotic regret scales as $(p(1-p))^2$ with respect to population parameter $p$. This particular scaling arises because the regret is roughly proportional to the second moment of the number of matches of $0$-$1$ type in the initial random matching. Thus, the asymptotic regret of the greedy Bayes algorithm matches the lower bound in Table~\ref{tab:lb} for the CES $0<a\leq 1$ function up to a constant factor. This is because the CES $0<a\leq 1$ function satisfies the constant improvement property. 

Observe that the worst-case asymptotic regret is achieved for a balanced population case (i.e. when $p = 1/2$) and that the asymptotic regret decreases as the population is less balanced (i.e. $p$ is further away from $1/2$). Unlike to maximum value function case, the regret is symmetric with respect to population parameter $p$ around $1/2$. This tells us that searching for an optimal matching is equally difficult for the case when $p=\gamma$ and when $p = 1-\gamma$ for the greedy Bayes algorithm. This is intuitive given what information is extracted from each pair examination. Observe further that the asymptotic regret  is proportional to $p^2 n^2$ for small $p$ case and is proportional to $(1-p)^2 n^2$ for large $p$ case. The asymptotic regret increases with parameter $a$ on $(0,1]$ and it approaches zero as $a\uparrow 1$. This is intuitive because when $a = 1$, by Lemma~\ref{lm:cesop1}, any matching is an optimal matching. In Figure~\ref{fig:regret-ces-complements}, we show how the asymptotic regret depends on the population parameter $p$ for several different values of parameter $a$.

\begin{figure}[t]
\begin{center}
\includegraphics[width=7cm]{regret-ces-supplements.png}
\caption{The asymptotic normalized regret for the CES function (for some values $0 < a \leq 1$) in the limit for large number of nodes $n$, versus population parameter $p$.}
\label{fig:regret-ces-supplements}
\end{center}
\end{figure}

\paragraph{Complements case $a > 1$}

In contrast to the substitutes case, the total value of any two pairs of $0$-$1$ type is larger than the total value of two pairs of $0$-$0$ and $1$-$1$ type. The following lemma gives a necessary and sufficient condition for a matching to be an optimal matching. 

\begin{lemma} For value function $\f$ being the CES function with $a > 1$, a matching is optimal if, and only if, the matching does not contain a pair of $0$-$0$ and a pair of $1$-$1$ type.
\label{lm:cesopt2}
\end{lemma}

The greedy Bayes algorithm selects two pairs of $0$-$0$ and $1$-$1$ type one after other, and re-matches each of them to create two pairs of $0$-$1$ type. The algorithm terminates when the matching does not contain a pair of $0$-$0$ type and a pair of $1$-$1$ type. Note that in each round, the greedy Bayes algorithm guarantees to decrease the instantaneous regret for at least $2-2^{1/a}$ over the next two rounds. Thus, CES $a > 1$ value function satisfies the constant improvement property.    

\begin{theorem} 
For CES value function $\f$ with $a > 1$, the regret of greedy Bayes algorithm satisfies
$$
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) \sim \frac{1}{4}(2-2^{1/a})\min\{p,1-p\}^4 n^2, \hbox{ for large } n.
$$
\label{thm:ces2}
\end{theorem}

Proof of Theorem~\ref{thm:ces2} is provided in Appendix~\ref{app:ces2}. The proof is simple. The number of examinations of two pairs of $0$-$0$ and $1$-$1$ type corresponds to the minimum of the number of pairs of $0$-$0$ type and the number of pairs $1$-$1$ type in the initial random matching. Each examination results in finding two pairs of $0$-$0$ and $1$-$1$ type. The examinations are completed as soon as there are no two pairs of $0$-$0$ and $1$-$1$ type left. The expected regret is computed by simple accounting for the expected instantaneous regret accrued in each step. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=7cm]{regret-ces-complements.png}
\caption{The asymptotic normalized regret for the CES function (for some values $a > 1$) in the limit for large number of nodes $n$, versus population parameter $p$.}
\label{fig:regret-ces-complements}
\end{center}
\end{figure}

The asymptotic regret scales as $\min\{p,1-p\}^4$ with the population parameter $p$. This particular scaling arises because the asymptotic regret is essentially determined by the instantaneous regret incurred in the initial random matching. This is because the CES $a>1$ value function satisfies the constant improvement property. Observe that the asymptotic regret has qualitatively similar dependence on the population parameter $p$ as for the case of substitutes. The worst-case is achieved for the balanced population case, i.e. when $p=1/2$, and the asymptotic regret decreases as the population becomes less balanced, i.e. the further away $p$ is from $1/2$. The asymptotic regret is symmetric around $1/2$ with respect to the value of the population parameter $p$. Note that the asymptotic regret scales proportionally to $p^4 n^2$ for small $p$ and it scales proportionally to $(1-p)^4 n^2$ for small $1-p$. Observe that the scaling is faster with $p$ and $1-p$ in the two limit cases than for the case of substitutes. This is intuitive because there are fewer pairs to be examined in the case of complements---proportional to the number of $0$-$1$ type pairs in the initial random matching, as opposed to the minimum between the number of $0$-$0$ type pairs and the number of $1$-$1$ type pairs in the initial random matching in the case of substitutes. The asymptotic regret has a factor $2-2^{1/a}$ which corresponds to the reduction of the instantaneous regret when re-matching two pairs of $0$-$0$ and $1$-$1$ type to two pairs of $0$-$1$ type. In the limit as $a \downarrow 1$ this factor goes to $0$ as diminishing gains are accrued from re-matching. On the other hand, when $a$ goes to infinity, the value accrued from a re-matching is $1$.


\subsection{Conclusion}
\label{sec:conc}




\subsection{Mathematical background}

\subsubsection{Differential equation approximation}

Here we provide background results on differential equation approximation for discrete random processes by \cite{Wormald95}, which we use in the proof of Theorem~\ref{thm:max}.

Consider a discrete random process on probability space $\Omega$, denoted by $X_0, X_1, \ldots$, where each $X_t$ takes values in some set $S$. We use ${\mathcal F}_t$ to denote $(X_0, X_1, \ldots, X_t)$, the history of the process up to time $t$. For a function $y$ of history ${\mathcal F}_t$, random variable $y({\mathcal F}_t)$ is denoted by $Y_t$. 

We consider a sequence $\Omega_n$, $n = 1,2, \ldots$ of random processes. For a random variable $X$, we say $X = o(f(n))$ always if 
$$
\max\{x: \P[X=x]\neq 0\} = o(f(n)).
$$
An event is said to hold \emph{almost surely} if its probability in $\Omega_n$ is $1-o(1)$. Let $S_n^+$ denote the set of all functions $f_n (x_0, x_1,\ldots,x_t)$ where each $x_i \in S_n$, for $t\geq 0$. 

A function $f:\reals^d\rightarrow \reals$ is said to satisfy a Lipschitz condition on $D\subseteq \reals^d$ if there exists a constant $L > 0$ such that $|f(x)-f(y)|\leq L ||x-y||_1$ for all $x$ and $y$ in $D$.

Let $d$ be a fixed positive integer. For $i \in [d] = \{1,\ldots, d\}$, let
$$
y^{(i)} : \cup_n S_n^+\rightarrow \reals
$$
and $f_i: \reals^{d+1}\rightarrow \reals$ be such that for some constant $C$ and all $i\in [d]$,
$$
|y^{(i)}({\mathcal F}_t)| \leq Cn \hbox{ for all } {\mathcal F}_t \in S_n^+ \hbox{ for all } n.
$$
Assume that for some sequence $m(n)$, the following conditions hold:
\begin{enumerate}
\item[(C1)] there is a constant $C'$ such that for all $t< m(n)$ and all $i\in [d]$, it holds always,
$$
|Y^{(i)}_{t+1}-Y^{(i)}_t|\leq C'.
$$
\item[(C2)] for all $i\in [d]$ and uniformly over $t < m(n)$, it holds always,
$$
\E[Y^{(i)}_{t+1}-Y^{(i)}_t \mid {\mathcal F}_t] = f_i\left(\frac{t}{n}, \frac{Y_t^{(1)}}{n}, \ldots, \frac{Y^{(d)}_t}{n}\right) + o(1).
$$
\item[(C3)] for all $i\in [d]$, $f_i$ is continuous and satisfies a Lipschitz condition on $D$ where $D$ is some bounded connected open set containing the intersection of $\{(t,y^{(1)}, \ldots, y^{(d)}): t\geq 0\}$ with some neighborhood of $\{(0, y^{(1)}, \ldots, y^{(d)}): \P[\cap_{i\in [d]}\{Y^{(i)}_0 = y^{(i)}n\}]\neq 0 \hbox{ for some } n\}$.
\end{enumerate}

\begin{theorem}[\cite{Wormald95}] Assume that conditions (C1)-(C3) hold. Then, 
\begin{enumerate}
\item For $(0,\hat{x}^{(1)}, \ldots, \hat{x}^{(d)})\in D$, the system of differential equations
$$
\frac{d}{dt}x_i(t) = f_i(t,x_1(t), \ldots, x_d(t)), \hbox{ for } i\in [d]
$$
has a unique solution in $D$ for all $x_i:\reals\rightarrow \reals$ such that
$$
x_i(0) = \hat{x}^{(i)} \hbox{ for } i\in [d]
$$
and which extends to points arbitrarily close to the boundary of $D$.
\item The following holds almost surely
$$
Y^{(i)}_t = n x_i(t/n) + o(n)
$$
uniformly for $0 \leq t \leq \min\{\sigma(n) n, m(n)\}$, for all $i\in [d]$, where $x_i(t)$ is the solution of the differential equation with $\hat{x}^{(i)}(0) = Y^{(i)}_0 / n$ and $\sigma(n)$ is the supremum of $t$ for which the solution of the differential equation can be extended.
\end{enumerate}
\label{thm:wormald}
\end{theorem}

\subsection{Proofs}

\subsubsection{Proof of Lemma~\ref{lm:lb}}

Let $\f$ be an arbitrary value function and $\alg$ be an arbitrary local switching adaptive matching algorithm for value function $\f$. Algorithm $\alg$ reduces the instantaneous regret in each round for at most some constant value $L > 0$. Recall that any adaptive matching algorithm selects random matching for initial matching because the prior distribution is non-informative for maximum value matching. 

Let $R_t^\alg$ denote the instantaneous regret in round $t$, for $t\geq 1$. Note that it holds 
$$
R_t^\alg \geq \max\{R_1 - L(t-1),0\}, \hbox{ for all } t\geq 1
$$
where $R_1$ denotes the instantaneous regret of initial random matching (we omit the subscript $\alg$ in $R_1$ because this instantaneous regret does not depend on $\alg$).

Hence, for any $T\geq \lfloor \E[R_1]/L\rfloor$,
\begin{eqnarray*}
\E\left[\sum_{t=1}^T R_t^\alg\right] 
&\geq & \sum_{t=1}^T\E[\max\{R_1-L(t-1),0\}]\\
&\geq & \sum_{t=1}^T\max\{\E[R_1]-L(t-1),0\}\\
&\geq & \sum_{t=0}^{\lfloor \E[R_1]/L\rfloor -1} (\E[R_1]-Lt)\\
&=& \E[R_1]\left\lfloor \frac{\E[R_1]}{L}\right\rfloor - L\frac{1}{2} \left(\left\lfloor\frac{\E[R_1]}{L}\right\rfloor-1\right)\left\lfloor\frac{\E[R_1]}{L}\right\rfloor\\
&\geq & \frac{L}{2}\left\lfloor\frac{\E[R_1]}{L}\right\rfloor^2
\end{eqnarray*}
where the second inequality is by Jensen's inequality. 

For any fixed $c\in (0,1/(2L))$, assume that $\E[R_1] \geq L/(1 - \sqrt{2c L})$. Then,
$
\E[R_1]/L-1\geq \sqrt{2cL}(\E[R_1]/L)
$
and, thus, it follows
$$
\frac{L}{2}\left\lfloor\frac{\E[R_1]}{L}\right\rfloor^2 
\geq \frac{L}{2}\left(\frac{\E[R_1]}{L}-1\right)^2
\geq  c\E[R_1]^2.
$$

\subsubsection{Regret for random matching}
\label{sec:rnd}

%\mv{*** TBD - at different places may need to impose conditions on $p$ such as $pn = \Omega(1)$ or $pn = \omega(1)$ and similarly for $1-p$. Note that Lemma~\ref{lm:lb} requires $\tilde{R}_w = \omega(1)$ which will require conditions on $p$ and $1-p$. ***}

Let $M$ be a random matching and let $N^{00}$, $N^{01}$ and $N^{11}$ denote the number of matches in $M$ of type $0$-$0$, $0$-$1$ and $1$-$1$, respectively. Let $\f$ be an arbitrary value function. Then, we have
$$
\E[\mu_{\f}(M)] = \f(0,0)\E[N^{00}] + \f(0,1)\E[N^{01}] + \f(1,1)\E[N^{11}].
$$
It follows that
$$
\E[\mu_{\f}(M)] = \frac{1}{2}\left(\f(0,0)(1-p)^2 + \f(0,1)2p(1-p) + \f(1,1)p^2\right)n.
$$

In the following we consider the instantaneous regret of random matching for different value functions $\f$.

\paragraph{Maximum value function} In this case, we have 
$$
\E[\mu_{\f}(M)] = \frac{1}{2}(1-(1-p)^2)n.
$$

Any optimal matching $M^*$ has a maximum possible number of $0$-$1$ type pairs and any remaining high-type nodes matched with high-type nodes. Let $N^1$ denote the number of high-type nodes in the given set of nodes. Then, conditional on $\{N_1=n_1\}$, we have
$$
\E[\mu_{\f}(M^*)\mid N_1 = n_1]=\frac{1}{2}\min\left\{2n_1,n\right\}.
$$
This is because if $n_1\leq n/2$, then every high-type node is matched is with a low-type node yielding the total value of $n_1$, and, otherwise, if $n_1 > n/2$, then $n-n_1$ high-type nodes are matched with low-type nodes and the remaining $n_1-(n-n_1)$ high-type nodes are matched with high-type nodes, yielding the total value $(n-n_1) + (1/2)(n_1 -(n-n_1)) = n/2$. 

It follows that the expected weight of an optimal matching is
$$
\E[\mu_{\f}(M^*)] = \frac{1}{2}\E[\min\{2N_1,n\}]% \sim \min\left\{p,\frac{1}{2}\right\}n \hbox{ for large } n.
$$

Hence, we have
$$
\tilde{R}_w = \E[\mu_{\f}(M^*)]-\E[\mu_{\f}(M)] %
= \E\left[\min\left\{\frac{N_1}{n}-p + \frac{1}{2}p^2, \frac{1}{2}(1-p)^2\right\}\right]n.
%\sim \frac{1}{2}\min\{p,1-p\}^2n, \hbox{ for large } n.
$$
Since, for any real number $a$, $x\mapsto \min\{x,a\}$ is a concave function, by Jensen's inequality and $\E[N_1/n]-p = 0$, we have
$$
\tilde{R}_w \leq \frac{1}{2}\min\{p,1-p\}^2 n.
$$

We next show that it holds
$$
\tilde{R}_w \geq \frac{1}{2}\min\{p,1-p\}^2 n (1-o(1))
$$
provided that 
$$
\frac{p}{\log(1/p)^{1/4}} = \omega\left(\frac{1}{(c_n^2 n)^{1/4}}\right),
$$
and
$$
1-p = \omega\left(e^{-\frac{1}{2^6}c_n^2 n}\right)
$$
where $c_n$ is any sequence such that $c_n = o(1)$. Hence, under these conditions, 
$$
\tilde{R}_w \sim \frac{1}{2}\min\{p,1-p\}^2 n, \hbox{ for large } n.
$$

By Hoeffding's inequality,
$$
\Pr\left[\frac{N_1}{n}-p < -c_n \frac{1}{2}p^2\right]\leq e^{-\frac{1}{2}c_n^2 p^4 n}.
$$
It follows
\begin{eqnarray*}
\tilde{R}_w &=& \E\left[\min\left\{\frac{N_1}{n}-p + \frac{1}{2}p^2, \frac{1}{2}(1-p)^2\right\}\right]n\\
&\geq & \min\left\{(1-c_n)\frac{1}{2}p^2, \frac{1}{2}(1-p)^2\right\}n\left(1-e^{-\frac{1}{2}c_n^2 p^4 n}\right) - p e^{-\frac{1}{2}c_n^2 p^4 n}\\
& \geq & \frac{1}{2}\min\{p,1-p\}^2 n \left((1-c_n) \left(1-e^{-\frac{1}{2}c_n^2 p^4 n}\right)-2\max\left\{\frac{1}{p}, \frac{p}{(1-p)^2}\right\}e^{-\frac{1}{2}c_n^2 p^4 n}\right).
\end{eqnarray*}

Under conditions $c_n = o(1)$ and $p/\log(1/p)^{1/4} = \omega(1/(c_n^2 n)^{1/4})$, it clearly holds
$$
(1-c_n) \left(1-e^{-\frac{1}{2}c_n^2 p^4 n}\right) \geq 1-o(1).
$$
We next show that
$$
2\max\left\{\frac{1}{p}, \frac{p}{(1-p)^2}\right\}e^{-\frac{1}{2}c_n^2 p^4 n} 
= o(1).
$$

For the case when $p \leq 1/2$, we have
\begin{eqnarray*}
2\max\left\{\frac{1}{p}, \frac{p}{(1-p)^2}\right\}e^{-\frac{1}{2}c_n^2 p^4 n} & =& 2\frac{1}{p}e^{-\frac{1}{2}c_n^2 p^4 n}\\
&=& 2 e^{-\frac{1}{2}c_n^2 p^4 n (1-\log(1/p)/((1/2)c_n^2 p^4 n))}\\
&=& 2 e^{-\frac{1}{2}c_n^2 p^4 n (1-o(1))}\\
&=& o(1)
\end{eqnarray*}
where the two last relations hold by the condition $p/\log(1/p)^{1/4} = \omega(1/(c_n^2 n)^{1/4})$.


For the case when $p > 1/2$, 
\begin{eqnarray*}
2\max\left\{\frac{1}{p}, \frac{p}{(1-p)^2}\right\}e^{-\frac{1}{2}c_n^2 p^4 n} &=& 
2\frac{p}{(1-p)^2} e^{-\frac{1}{2}c_n^2 p^4 n}\\
&\leq & 2 e^{-\frac{1}{2^5}c_n^2 n + 2\log\left(\frac{1}{1-p}\right)}.
\end{eqnarray*}

The right-hand side in the last inequality is $o(1)$ if, and only if, 
$$
\frac{1}{2^6}c_n^2 n + \log\left(\frac{1}{1-p}\right) \rightarrow \infty \hbox{ as } n \rightarrow \infty, 
$$
i.e.
$$
1-p = \omega\left(e^{-\frac{1}{2^6}c_n^2 n}\right).
$$


\paragraph{Minimum value function} In this case, we have
$$
\E[\mu_{\f}(M)] = \frac{1}{2}p^2 n.
$$

Any optimal matching has maximum number of $1$-$1$ type pairs. Hence, we have
$$
\E[\mu_{\f}(M^*)] = \E\left[\left\lfloor\frac{N_1}{2}\right\rfloor\right]. 
$$

We next show that the regret of random matching satisfies
$$
\tilde{R}_{\f} = \E[\mu_{\f}(M^*)] - \E[\mu_{\f}(M)] = \frac{1}{2}p(1-p)n (1-o(1))
$$
provided that $p = \omega(1/n)$ and $1-p=\omega(1/n)$.


The regret of random matching has the following upper bound,
$$
\tilde{R}_{\f} = \E[\mu_{\f}(M^*)] - \E[\mu_{\f}(M)] \leq \frac{1}{2}pn - \frac{1}{2}p^2 n = \frac{1}{2}p(1-p)n
$$
and the following lower bound,
$$
\tilde{R}_{\f} = \E[\mu_{\f}(M^*)] - \E[\mu_{\f}(M)] \geq \frac{1}{2}pn - 1 - \frac{1}{2}p^2 n = \frac{1}{2}p(1-p)n - 1 = \frac{1}{2}p(1-p)n(1-o(1))
$$
where the last relation holds under conditions $p = \omega(1/n)$ and $1-p=\omega(1/n)$.

\paragraph{XOR value function} In this case, we have
$$
\E[\mu_{\f}(M)]= p(1-p)n.
$$

Any optimal matching maximizes the number of matches between nodes of different type. Hence, we have
$$
\E[\mu_{\f}(M^*)] = \E\left[\min\left\{N_1, n-N_1\right\}\right].
$$

We have
$$
\tilde{R}_{\f} = \E\left[\min\left\{\left(\frac{N_1}{n}-p\right)+p^2,-\left(\frac{N_1}{n}-p\right)+(1-p)^2\right\}\right].
$$

In the case when $p$ is a fixed constant, then we have
$$
\tilde{R}_{\f} \sim \min\{p,1-p\}^2 n \hbox{ for large } n.
$$

By Jensen's inequality, we have
$$
\tilde{R}_{\f} \leq \min\{p,1-p\}^2 n.
$$

We next show a lower bound on $\tilde{R}_{\f}$ when either $p = o(1)$ or $1-p=o(1)$. We first consider the case when $p<1/2$ and $p = o(1)$. Function $x\mapsto \min\{x+p^2,-x+(1-p)^2\}$ is increasing in $x$, for $x\leq 1/2-p$. By Hoeffding's inequality $\Pr[N_1/n-p<-c_n p^2]\leq e^{-2c_n^2 p^4 n}$. It follows
\begin{eqnarray*}
&& \E\left[\min\left\{\left(\frac{N_1}{n}-p\right)+p^2, -\left(\frac{N_1}{n}-p\right) + (1-p)^2\right\}\right]\\
& \geq & \min\{(1-c_n)p^2, c_n p^2 + (1-p)^2\}(1-e^{-2c_n^2 p^4 n}) + \min\{-p + p^2, p + (1-p)^2\}e^{-2c_n^2 p^4 n}\\
& \geq & (1-c_n)p^2 (1-e^{-2c_n^2 p^4 n}) - p e^{-2c_n^2 p^4 n}\\
& = & p^2 \left((1-c_n)(1-e^{-2c_n^2 p^4 n}) - \frac{1}{p}e^{-2c_n^2 p^4 n}\right)\\
&=& p^2 (1-o(1))
\end{eqnarray*}
where the last relation holds under condition $p/\log(1/p)^{1/4} = \omega(1/(c_n^2 n)^{1/4})$. 

We next consider the case when $p > 1/2$ and $1-p = o(1)$. Function $x\mapsto \min\{x+p^2, -x + (1-p)^2\}$ is decreasing in $x$, for $x\geq 1/2 - p$. By Hoeffding's inequality, $\Pr[N_1/n-p>c_n(1-p)^2]\leq e^{-2c_n^2(1-p)^4 n}$. It follows 
\begin{eqnarray*}
&& \E\left[\min\left\{\left(\frac{N_1}{n}-p\right)+p^2, -\left(\frac{N_1}{n}-p\right) + (1-p)^2\right\}\right]\\
& \geq & \min\{c_n(1-p)^2 + p^2, (1-c_n)(1-p)^2\}(1-e^{-2c_n^2 (1-p)^4 n}) + \min\{1-p+p^2, -p(1-p)\} e^{-2c_n^2 (1-p)^4 n}\\
& \geq & (1-c_n)(1-p)^2(1-e^{-2c_n^2 (1-p)^4 n}) - (1-p) e^{-2c_n^2 (1-p)^4 n}\\
& = & (1-p)^2 \left((1-c_n)(1-e^{-2c_n^2 (1-p)^4 n}) - \frac{1}{1-p} e^{-2c_n^2 (1-p)^4 n}\right)\\
&=& (1-p)^2 (1-o(1))
\end{eqnarray*}
where the last relation holds under condition $(1-p)/\log(1/(1-p))^{1/4} = \omega(1/(c_n^2 n)^{1/4})$. 

We have shown that
$$
\tilde{R}_{\f} \geq \min\{p,1-p\}^2 n (1-o(1))
$$
under conditions $p/\log(1/p)^{1/4} = \omega(1/(c_n^2 n)^{1/4})$ and $(1-p)/\log(1/(1-p))^{1/4} = \omega(1/(c_n^2 n)^{1/4})$.

\paragraph{NXOR value function} In this case, we have
$$
\E[\mu_{\f}(M)] = \frac{1}{2}((1-p)^2 + p^2)n.
$$
Any optimal matching maximizes the number of matches between nodes of the same type and value is gained only from these matches. Hence, we have
$$
\E[\mu_{\f}(M^*)] = \E\left[\left\lfloor \frac{N_1}{2}\right\rfloor\right] + \E\left[\left\lfloor\frac{n-N_1}{2}\right\rfloor\right].
$$

We next show that the regret of random matching satisfies
$$
\tilde{R}_{\f} = \E[\mu_{\f}(M^*)] - \E[\mu_{\f}(M)] = p(1-p)n (1-o(1))
$$
provided that $p = \omega(1/n)$ and $1-p=\omega(1/n)$.

The regret of random matching has the following upper bound,
$$
\tilde{R}_{\f} = \E[\mu_{\f}(M^*)] - \E[\mu_{\f}(M)] \leq \frac{1}{2}pn + \frac{1}{2}(1-p)n - \frac{1}{2}((1-p)^2 + p^2)n = p(1-p)n
$$
and the following lower bound,
\begin{equation*}
\begin{split}
        \tilde{R}_{\f} 
        &= \E[\mu_{\f}(M^*)] - \E[\mu_{\f}(M)] \\
        &\leq \frac{1}{2}pn - 1 + \frac{1}{2}(1-p)n - 1 - \frac{1}{2}((1-p)^2 + p^2)n \\
        &= p(1-p)n - 2 \\ 
        &= p(1-p)n (1-o(1))
\end{split}
\end{equation*}

where the last relation holds under conditions $p=\omega(1/n)$ and $1-p = \omega(1/n)$.

\paragraph{CES value function} Assume that $\f$ is the CES function for some $a > 0$. In this case, we have
$$
\E[\mu_{\f}(M)] = \left(p(1-p) + 2^{1/a-1} p^2\right)n.
$$

We next separately consider the two cases when either $0< a\leq 1$ (supplements) or $a > 1$ (complements). First, consider the case of supplements, i.e. $0<a\leq 1$. In this case, an optimal matching has the maximum possible number of $1$-$1$ type matches. Hence, we have
$$
\E[\mu_{\f}(M^*)\mid N_1 = n_1] = 2^{1/a} \left\lfloor \frac{n_1}{2}\right\rfloor + \left(n_1 - 2\left\lfloor \frac{n_1}{2}\right\rfloor\right).
$$
It follows
$$
\E[\mu_{\f}(M^*)] = (2^{1/a}-2)\E\left[\left\lfloor\frac{N_1}{2}\right\rfloor\right] + \E[N_1].
%\sim 2^{1/a-1}pn \hbox{ for large } n.
$$
We have the following upper bound,
$$
\E[\mu_{\f}(M^*)] \leq (2^{1/a}-2)\frac{1}{2}pn + pn = 2^{1/a-1} pn.
$$
Hence, we have
$$
\tilde{R}_w \leq (2^{1/a}-1)p(1-p)n.
$$
We have the following lower bound,
$$
\E[\mu_{\f}(M^*)] \geq (2^{1/a}-2)\frac{1}{2}pn - (2^{1/a}-2) + pn = 2^{1/a-1} pn - (2^{1/a}-2).
$$
Hence, we have
$$
\tilde{R}_w \geq (2^{1/a}-1)p(1-p)n - (2^{1/a}-2) = (2^{1/a}-1)p(1-p)n (1-o(1))
$$
where the last relation holds under conditions $p = \omega(1/n)$ and $1-p=\omega(1/n)$.

We next consider the case of complements, i.e. $a > 1$. In this case, an optimal matching maximizes the number of $0$-$1$ type pairs. Hence, we have
$$
\E[\mu_{\f}(M^*)\mid N_1 = n_1] = n_1 \ind_{\{n_1\leq n/2\}} + \left(n-n_1 + 2^{1/a}\left\lfloor \frac{2n_1-n}{2}\right\rfloor\right)\ind_{\{n_1 > n/2\}}.
$$
This is because when $n_1 \leq n/2$ then all high-type nodes are matched with low-type nodes yielding the total value of $n_1$, and when $n_1 > n/2$ then $n-n_1$ high-type nodes are matched with low-type nodes and the remaining $2n_1-n$ high-type nodes are matched among themselves. From the above expression, we have
\begin{eqnarray*}
\E[\mu_{\f}(M^*)] = \E[\min\{N_1, n-N_1\}] + 2^{1/a-1}\E[\max\{2N_1-n,0\}].
%\\
%&\sim & \min\{p,1-p\}n + 2^{1/a-1}\max\{2p-1,0\} n, \hbox{ for large } n.
\end{eqnarray*}

It is readily observed that for any fixed value of $p$,
$$
\tilde{R}_{\f} \sim (1-2^{1/a-1})\min\{p,1-p\}^2 n \hbox{ for large } n. 
$$

We next consider the case when either $p=o(1)$ or $1-p = o(1)$. 


We first show a lower bound on the regret. By Jensen's inequality, we have
$$
\E[\mu_{\f}(M^*)] \geq \E[\min\{N_1, n-N_1\}] + 2^{1/a-1}\max\{2p-1,0\}n.
$$

Hence, 
$$
\tilde{R}_{\f} \geq \E[\min\{N_1, n-N_1\}] - p(1-p)n - 2^{1/a-1}\min\{p^2, (1-p)^2\}n.
$$

%Note that
%$$
%\E[\min\{N_1, n-N_1\}] - p(1-p)n = \E\left[\min\left\{\left(\frac{N_1}{n}-p\right)+p^2, -\left(\frac{N_1}{n}-p\right) + (1-p)^2\right\}\right]n.
%$$

From the proof of the lower bound for regret of random matching for XOR function, we have
$$
\E[\min\{N_1,n-N_1)]\geq \min\{p,1-p\}^2 n (1-o(1))
$$
under conditions under conditions $p/\log(1/p)^{1/4} = \omega(1/(c_n^2 n)^{1/4})$ and $(1-p)/\log(1/(1-p))^{1/4} = \omega(1/(c_n^2 n)^{1/4})$.

Hence, it follows
$$
\tilde{R}_{\f} \geq (1-2^{1/a}-1)\min\{p,1-p\}^2 n (1-o(1))
$$
under conditions $p/\log(1/p)^{1/4} = \omega(1/(c_n^2 n)^{1/4})$ and $(1-p)/\log(1/(1-p))^{1/4} = \omega(1/(c_n^2 n)^{1/4})$.

We next show an upper bound on the regret. By Jensen's inequality,
$$
\E[\mu(M^*)]\leq \min\{p,1-p\}n + 2^{1/a-1} \E[\max\{2N_1-n,0\}].
$$
Hence,
$$
\tilde{R}_{\f} \leq \min\{p,1-p\}^2 n + 2^{1/a-1}\left(\E\left[\max\left\{2\frac{N_1}{n}-1,0\right\}\right]-p^2\right)n.
$$
Next, note that
$$
\E\left[\max\left\{2\frac{N_1}{n}-1,0\right\}\right]-p^2 = \E\left[\max\left\{2\left(\frac{N_1}{n}-p\right)-(1-p)^2,-p^2\right\}\right].
$$
By Hoeffding's inequality, $\Pr[N_1/n-p > c_n(1-p)^2/2]\leq e^{(1/2)c_n^2(1-p)^4 n}$. Hence, it follows
\begin{eqnarray*}
&& \E\left[\max\left\{2\left(\frac{N_1}{n}-p\right)-(1-p)^2,-p^2\right\}\right] \\
&\leq & \max\{-(1-c_n)(1-p)^2,-p^2\}(1-e^{-(1/2)c_n^2(1-p)^4 n}) + \max\{1-p^2,-p^2\}e^{-(1/2)c_n^2(1-p)^4 n}\\
&\leq & -(1-c_n)\min\{(1-p)^2,p^2\}(1-e^{-(1/2)c_n^2(1-p)^4 n}) + e^{-(1/2)c_n^2(1-p)^4 n}\\
&= & -\min\{p,1-p\}^2\left((1-c_n)(1-e^{-(1/2)c_n^2(1-p)^4 n}) - \frac{1}{\min\{p,1-p\}^2}e^{-(1/2)c_n^2 (1-p)^4 n}\right)\\
&=& -\min\{p,1-p\}^2 (1-o(1))
\end{eqnarray*}
where the last relation holds under conditions $(1-p)/\log(1/(1-p))^{1/4} = \omega(1/(c_n^2 n)^{1/4})$ and $p = \omega(e^{-\kappa c_n^2 n})$, for any constant $\kappa \in (0,1)$.

Putting the pieces together, we have
$$
\tilde{R}_{\f} \leq (1-2^{1/a-1})\min\{p, 1-p\}^2 n (1+o(1))
$$
under conditions $(1-p)/\log(1/(1-p))^{1/4} = \omega(1/(c_n^2 n)^{1/4})$ and $p = \omega(e^{-\kappa c_n^2 n})$, for any constant $\kappa \in (0,1)$.


\subsubsection{Proof of Theorem~\ref{thm:max}}
\label{app:max}

%\mv{*** Note that appying Wormald's theorem may require some conditions on $p$, e.g. $p$ being a constant ***.}
%\jy{checked. It holds for all $p$ being constant in $(0, 1)$ or $p=1-o(1)$ or $p=o(1)$.}

For each round $t\geq 0$, let $S_t$ be the number of matches known to be of $0$-$0$ type, $U_t$ be the number of matches known to be of either $0$-$1$ or $1$-$1$ type, and $K_t$ be the number of matches known to be of $0$-$1$ type. 

Let $N_1$ be the number of type $1$ items in round $1$. Let $U_t^{01}$ be the number of matches of $0$-$1$ type and $U_t^{11} := U_t - U_t^{01}$. The following equations hold, for every $t\geq 0$,
\begin{eqnarray}
U_t^{01} + U_t^{11} &=& U_t \label{equ:sum0}\\
S_t + U_t + K_t &=& \frac{n}{2}\label{equ:sum1}\\
U^{11}_t + U_t + K_t &=& N_1.\label{equ:sum2}
\end{eqnarray}

By the law of large numbers, the following limits hold almost surely,
\begin{eqnarray}
\lim_{n\rightarrow \infty} \frac{1}{n}N_1 &=& p\label{equ:n1}\\
\lim_{n\rightarrow \infty} \frac{2}{n}U_1^{11} &=& p^2\label{equ:u111}\\
\lim_{n\rightarrow \infty} \frac{2}{n}S_1 &=& (1-p)^2\label{equ:s1}\\
\lim_{n\rightarrow \infty} \frac{2}{n}U_1 &=& 1-(1-p)^2.\label{equ:u1}
\end{eqnarray}

For any $p\in (0,1)$, $S_1 \wedge U_1 > 0$ almost surely.
% Initially, in round $t=1$, the matching is a random matching, for which it holds $\P[\{S_1=0\}\cup \{U_1=0\}] = [1-(1-p)^2]^{n/2} + [(1-p)^2]^{n/2} = o(1)$. \mv{*** This requires $(1-p)^2 n = \omega(1)$ and $pn = \omega(1)$. ***} 
Hence, in what follows we condition on $\{S_1>0\}\cap \{U_1>0\}$. 

The system dynamics is according to the Markov chain $\{X_t\}_{t\geq 0}$ where $X_t = (S_t, U_t^{01}, U_t^{11},K_t)$ with transition probabilities given as follows
\begin{eqnarray}
S_{t+1} &=& S_t - \xi_t \ind_{\{S_t\wedge U_t > 0\}}\label{equ:mc-s}\\
U^{11}_{t+1} &=&   U^{11}_t - \xi_t \ind_{\{S_t\wedge U_t > 0\}}\label{equ:mc-u11}\\
U^{01}_{t+1} &=&  U^{01}_t - (1-\xi_t) \ind_{\{S_t\wedge U_t > 0\}}\label{equ:mc-u01}\\
K_{t+1} &=& K_{t} + (1+\xi_t )\ind_{\{S_t\wedge U_t > 0\}}\label{equ:mc-k}
\end{eqnarray}
where $\xi_t$ is a Bernoulli random variable with mean $U^{11}_t/U_t$ under condition $U_t > 0$.

Conditional on $\{N_1 = n_1\}$, the expected reward of an optimal matching is 
$$
\mu^* = \frac{n_1 + \min\{n_1, n-n_1\}}{2}.
$$
The instantaneous reward at round $t$ is 
$$
\mu_t = U_t + K_t. %+ \xi_t \ind_{\{S_t\wedge U_t > 0\}}.
$$
%\jy{***why $\xi_t \ind_{\{S_t\wedge U_t > 0\}}$ ***}

Hence, the instantaneous regret $R_t$ at round $t$ is equal to
\begin{equation}
R_t = U^{11}_{t} + \min\left\{\frac{n}{2} - N_1, 0\right\}.
\label{equ:rt}
\end{equation}

The algorithm terminates at the stopping time $\tau$ defined as
$$
\tau = \min\{t > 1\mid  S_t = 0 \hbox{ or } U_t = 0\}.
$$
Note that $\tau$ satisfies, with probability $1$,
$$
S_1\wedge U_1 + 1\leq \tau \leq U_1 + 1.
$$
To see this, note that from (\ref{equ:mc-s}), $S_t \geq S_1 - (t-1)$. Hence, $S_t = 0$ implies $t \geq S_1 + 1$. Similarly, from (\ref{equ:mc-u11}) and (\ref{equ:mc-u01}), $U_t \geq U_1 - (t-1)$, hence $U_t = 0$ implies $t \geq U_1 + 1$. From this, it follows that $\tau \geq S_1 \wedge U_1 + 1$. Now, for the upper bound, suppose first that $S_\tau \geq U_\tau = 0$. Since in this case $U_\tau = U_1 - (\tau-1)$, it follows that $\tau = U_1 + 1$. Otherwise, if $0 = S_\tau < U_\tau$, it follows that $\tau \leq U_1 + 1$, which establishes the upper bound.

From (\ref{equ:sum0}), (\ref{equ:mc-u11}) and (\ref{equ:mc-u01}), for all $t\geq 1$, $U_{t+1} = U_t - \ind_{\{S_t \wedge U_t > 0\}}$. Hence, for all $t\geq 1$,
$$
U_{t} = U_1 - (t-1)\ind_{\{S_t\wedge U_t > 0\}} - \tau \ind_{\{S_t\wedge U_t = 0\}}.
$$

From (\ref{equ:mc-s}) and (\ref{equ:mc-u11}), for all $t\geq 1$, $S_t - U^{11}_t = S_1 - U^{11}_1$. Hence, $S_t > 0$ is equivalent to $U^{11}_t > U^{11}_1 - S_1$.

It follows that the system evolves according to a one-dimensional time-inhomogenous Markov chain $\{U^{11}_t\}_{t\geq 1}$ with transition probabilities given as, for $t \leq u_1$,

$$
\P_1[U^{11}_{t+1} = u -1 \mid U^{11}_t = u ] = \frac{u}{u_1-(t-1)}\ind_{\{u > u^{11}_1 - s_1\}}
$$
and
\begin{eqnarray*}
\P_1[U^{11}_{t+1} = u \mid U^{11}_t = u ] 
= 1-\P_1[U^{11}_{t+1} = u -1 \mid U^{11}_t = u ]
\end{eqnarray*}
and, for $ t > u_1$,
$$
\P_1[U^{11}_{t+1} = u \mid U^{11}_t = u] = 1.
$$

For all $1\leq t \leq u_1$, we have
$$
\E_1[U^{11}_{t+1}] = \E_1[U^{11}_t] - \E_1\left[\frac{U^{11}_t}{U_t} \ind_{\{U^{11}_t > u^{11}_1 - s_1\}}\right].
$$
and, for $t > u_1$,
$$
\E_1[U^{11}_{t+1}] = \E_1[U^{11}_t].
$$

% In the following we consider two cases with respect to the sign of $u_1^{11}-s_1$.
In the following we consider two cases with respect to the sign of $p-1/2$.

\noindent {\bf Case 1}: $p\leq 1/2$. From \eqref{equ:n1}, \eqref{equ:u111} and \eqref{equ:n1}, it holds, almost surely 
$$
U_1^{11} \leq S_1, \quad N_1 \leq \frac{n}{2}.
$$
By \eqref{equ:rt}, it holds, almost surely,
$$
R_t = U^{11}_t.
$$
In this case, we have
$$
\E_1\left[\frac{U^{11}_t}{U_t} \ind_{\{U^{11}_t > u^{11}_1 - s_1\}}\right] = \E_1\left[\frac{U^{11}_t}{U_t}\right] = \frac{1}{u_t}\E_1[U^{11}_t]
$$
and $u_t = u_1 -(t-1)$. Hence, for $1\leq t\leq u_1$, $\E_1[U^{11}_{t+1}] = \frac{u_{t+1}}{u_t}\E_1[U^{11}_t]$, and, thus, expanding this recurrence, we obtain
$$
\E_1[U^{11}_{t}] = \frac{u_t}{u_1}u^{11}_1.
$$
It follows that for all $t\geq 1$,
\begin{equation}
\E_1[U^{11}_{t}] = \left(1 - \frac{t-1}{u_1}\right)^+u^{11}_1
\label{equ:e11t}
\end{equation}
where $(\cdot)^+ = \max\{\cdot,0\}$.

We have, for $t\geq 1$,
\begin{eqnarray*}
\E_1[R_t] &=& \E_1[U^{11}_{t}] = \left(1 - \frac{t-1}{U_1}\right)^+U^{11}_1.
\end{eqnarray*}
Hence, we have
\begin{eqnarray*}
\E\left[\sum_{t=1}^{U_1 + 1} R_t \right] &=& \E\left[\sum_{t=1}^{U_1+1} \left(1 - \frac{t-1}{U_1}\right)^+U^{11}_1\right]\\
&=& \frac{1}{2}\E\left[U^{11}_1 \left(U_1 +1\right) \right]\\
&=& \frac{1}{2}\E[U^{11}_1 U_1] + \frac{1}{2}\E[U^{11}_1]\\
&=& \frac{1}{2}\E[\E[U^{11}_1\mid U_1] U_1] + \frac{1}{2}\E[U^{11}_1]\\
&=& \frac{1}{2}\frac{p^2}{1-(1-p)^2}\E[U_1^2] + \frac{1}{4}p^2 n\\
&=& \frac{1}{2}\frac{p^2}{1-(1-p)^2}\left((1-(1-p)^2)^2 \frac{n^2}{4} + \frac{n}{2}(1-(1-p)^2)(1-p)^2\right) + \frac{1}{4}p^2 n\\
&=& \frac{1}{8}(1-(1-p)^2)p^2 n^2 + \frac{1}{4}p^2 (1-p)^2 n + \frac{1}{4}p^2 n\\
&=& \frac{1}{8}(1-(1-p)^2)p^2 n^2 + \frac{1}{4}p^2(1+(1-p)^2) n\\
&=& \frac{1}{8}(1-(1-p)^2)p^2 n^2 (1+o(1))
%&=& \frac{1}{8} (1-(1-p)^2)p^2 n^2 + \jy{\frac{1}{4}p^2n}. 
\end{eqnarray*}
where the last relation holds under condition $p = \omega(1/n)$.

%When
%$$
%p > 1- \sqrt{1-\frac{2}{n}}
%$$
%the first term is the dominant term.

% \jy{---------------------Remove----------------------}

% \jy{By \eqref{equ:rt},
% \begin{eqnarray*}
% \E_1[R_t] &=& \E_1[U^{11}_{t+1}] + \min\{\frac{n}{2}-N_1,0\} = \left(1 - \frac{t}{u_1}\right)^+u^{11}_1+ \min\{\frac{n}{2}-N_1,0\} .
% \end{eqnarray*}
% }
% \jy{
% Hence we have
% \begin{eqnarray*}
% \E\left[\sum_{t=1}^{U_1 + 1} R_t \right] 
% &=& \E\left[\sum_{t=1}^{U_1 + 1} \E_1[R_t] \right]  \\
% &=& \E\left[\sum_{t=1}^{U_1+1} \left(1 - \frac{t}{U_1}\right)^+U^{11}_1\right]\\
% && + \E\left[(U_1+1)\min\left\{\frac{n}{2}-N_1,0\right\}\right]\\
% &\leq& \frac{1}{2}\E\left[U_1 U^{11}_1\right] + o(n^2)\\
% &\leq& \frac{1}{8} (1-(1-p)^2)p^2 n^2 + o(n^2). 
% \end{eqnarray*}
% }


\noindent {\bf Case 2}: $p>1/2$ From \eqref{equ:n1}, \eqref{equ:u111} and \eqref{equ:n1}, we have, almost surely, 
$$
U_1^{11} > S_1, \quad N_1 > \frac{n}{2}.
$$
By \eqref{equ:rt}
$$
R_t = U^{11}_t + \frac{n}{2} - N_1
$$


% $z := u_1^{11} -s_1 > 0$. By a simple comparison argument, we have, for all $t\geq 1$,
% $$
% \E_1[U^{11}_{t}] \geq \left(1 - \frac{t-1}{u_1}\right)^+u^{11}_1.
% $$
% To obtain an upper bound on $\E_1[U^{11}_t]$, we proceed as follows. 

% Since for $1\leq t\leq S_1 \wedge U_1$, $S_t \wedge U_t > 0$, with probability $1$, and in the present case $s_1 < u_1$, we have, for $1\leq t \leq s_1$,
% $$
% \E_1[U^{11}_{t}] = \left(1 - \frac{t-1}{u_1}\right)u^{11}_1.
% $$

% Note that
% \begin{eqnarray*}
% U^{11}_{t+1}\ind_{\{S_{t+1} > 0\}} &=& U^{11}_t \ind_{\{S_{t+1}>0\}} - \xi_t \ind_{\{S_t > 0\}}\ind_{\{S_{t+1}>0\}}.
% \end{eqnarray*}

% Note also
% \begin{eqnarray*}
% U^{11}_t \ind_{\{S_{t+1}>0\}} &=& U^{11}_t \ind_{\{S_{t+1}>0\}}\ind_{\{S_{t}>0\}}\\
% &=& U^{11}_t \ind_{\{S_{t}>0\}} - U^{11}_t \ind_{\{S_{t}>0\}} \ind_{\{S_{t+1}=0\}}\\
% &=& U^{11}_t \ind_{\{S_{t}>0\}} - (z+1) \ind_{\{S_{t}>0\}} \ind_{\{S_{t+1}=0\}}.
% \end{eqnarray*}

% Similarly, we have
% \begin{eqnarray*}
% \xi_t\ind_{\{S_t > 0\}}\ind_{\{S_{t+1}>0\}} &=& \xi_t \ind_{\{S_t > 0\}} - \xi_t \ind_{\{S_t > 0\}}\ind_{\{S_{t+1}=0\}}.
% \end{eqnarray*}

% Putting the pieces together, we have
% \begin{eqnarray*}
% U^{11}_{t+1}\ind_{\{S_{t+1} > 0\}} &=& [U^{11}_t-\xi_t] \ind_{\{S_{t}>0\}} - [(z+1)-\xi_t] \ind_{\{S_{t}>0\}}\ind_{\{S_{t+1}=0\}}.
% \end{eqnarray*}

% Taking expectation on both sides of the last equation, we have
% \begin{eqnarray*}
% \E_1[U^{11}_{t+1}\ind_{\{S_{t+1} > 0\}}] 
% &=& \frac{u_{t+1}}{u_t} \E_1[U^{11}_t \ind_{\{S_t>0\}}]  - (z+1) \frac{u_{t+1}}{u_t} \P_1[S_t > 0, S_{t+1} = 0].
% \end{eqnarray*}

% Note that
% $$
% \P_1[S_t > 0, S_{t+1} = 0] = \P_1[\tau = t+1].
% $$

% It follows that
% \begin{eqnarray*}
% \E_1[U^{11}_{t}\ind_{\{S_{t} > 0\}}] 
% &=& \frac{u_t}{u_1}u^{11}_1  - (z+1)\sum_{i=1}^{t-1} \frac{u_{t-i+1}}{u_i}\P_1[\tau = i+1].
% \end{eqnarray*}

% Now, since $\E_1[U^{11}_{t+1}] = \E_1[U^{11}_t] - \E_1[(U^{11}_t/U_t)\ind_{\{S_t > 0\}}]$, we have
% $$
% \E_1[U^{11}_t] = u^{11}_1 - \sum_{j=1}^{t-1}\frac{1}{u_j}\E_1[U^{11}_j\ind_{\{S_j > 0\}}].
% $$
% Hence, it follows
% \begin{eqnarray*}
% \E_1[U^{11}_t] &=& \left(1-\frac{t-1}{u_1}\right)u_1^{11} + (z+1)\sum_{j=1}^{t-1}\sum_{i=1}^{j-1} \frac{u_{j-i+1}}{u_j u_i}\P_1[\tau=i+1]
% \end{eqnarray*}
% which is equivalent to
% \begin{eqnarray*}
% \E_1[U^{11}_t] &=& \left(1-\frac{t-1}{u_1}\right)u_1^{11}  + (z+1)\sum_{i=1}^{t-2} a_i \P_1[\tau=i+1]
% \end{eqnarray*}
% where
% $$
% a_i = \frac{1}{u_i}\sum_{j=i+1}^{t-1} \frac{u_{j-i+1}}{u_j}.
% $$

% Note that
% \begin{eqnarray*}
% \P_1[\tau = t+1] &=& \E_1[\ind_{\{S_{t+1} = 0\}}\ind_{\{S_t > 0\}}]\\
% &=& \E_1\left[\frac{z+1}{U_t}\ind_{\{U^{11}_t = z+1\}}\right]\\
% &=& \frac{z+1}{u_t}\P_1[U^{11}_t =z+1].
% \end{eqnarray*}

We next establish a limit value of $U^{11}_t$ as $n$ goes to infinity, for $p > 1/2$ %\mv{*** Why is this condition here?***}\jy{solved.}
%% \jy{***Do not know where $p>1/2$ comes from ***} 
by applying Theorem~\ref{thm:wormald}. 

Condition (C1) holds because for all $t\geq 1$, it always holds,
$$
|U^{11}_{t+1} - U^{11}_t| \leq 1.
$$
Condition (C2) holds as follows 
% \jy{***Why this holds as Condition (2)***}
$$
\E[U^{11}_{t+1}-U^{11}_t\mid {\mathcal F}_t] = f(t/n,U^{11}_t/n)\ind_{\{U_t^{1,1}/n > \tilde{z}\}}
$$
where $U^{11}_1-S_1 = \tilde{z} n + o(n)$, and 
$$f(t,x) = -\frac{x}{\tilde{u}_1-t},$$ 
for $x > \tilde{z}$, where $u_1 = \tilde{u}_1 n + o(n)$ and $\tilde{u}_1 = \frac{1}{2}p(2-p)$.

{Hence, when $p\in (1/2, 1)$ is fixed,
$$
\E[U^{11}_{t+1}-U^{11}_t\mid {\mathcal F}_t] = -\frac{U^{11}_t/n}{\frac{1}{2}p(2-p)-t/n} + o(1),
$$
and, when $p=1-o(1)$,
$$
\E[U^{11}_{t+1}-U^{11}_t\mid {\mathcal F}_t] = -\frac{U^{11}_t/n}{\frac{1}{2}-t/n} + o(1).
$$
For condition (C3), we need to show that $f$ satisfies a Lipschitz condition on $D = \{(t,x): 0 \leq t < t^\star, 0 \leq x \leq 1\}$. Note that
\begin{eqnarray*}
|f(t,x)-f(t',x')|  &= & |f(t,x)-f(t',x)+f(t',x)-f(t',x')|\\
&\leq & \frac{|f(t,x)-f(t',x)|}{|t-t'|}|t-t'|+ \frac{|f(t',x)-f(t',x')|}{|x-x'|}|x-x'|\\
&\leq & L (|t-t'| + |x-x'|) 
\end{eqnarray*}
where
$$
L = \max_{(t,x)\in D} \left|\frac{\partial}{\partial t } f(t,x)\right| \vee \max_{(t,x)\in D}\left|\frac{\partial}{\partial x} f(t,x)\right|.
$$
Since $\partial f(x,t)/\partial t = x/(\tilde{u}_1 -t)^2$ and $\partial f(x,t)\partial x = -1/(\tilde{u}_1 - t)$, we have
$$
L = \frac{\tilde{u}^{11}_1}{(\tilde{u}_1-t^\star)^2} \vee \frac{1}{\tilde{u}_1-t^\star}
$$
where $t^\star$ is the unique positive value such that $u^{11}(t^\star) = \tilde{z}$. Note that
$$
t^\star = \left(1-\frac{\tilde{z}}{\tilde{u}^{11}_1}\right)\tilde{u}_1 = \frac{(1-(1-p)^2)(1-p)^2}{2p^2}
$$
and
$$
\tilde{u}_1 - t^\star = \frac{1-(1-p)^2}{p^2}\left(p-\frac{1}{2}\right).
$$

Next, consider the differential equation, 
$$
\frac{d}{dt}u^{11}(t) = f(t,u^{11}(t)), \hbox{ for } 0\leq t < t^\star.
$$
This differential equation has a unique solution which is given by
$$
u^{11}(t) = \left(1-\frac{t}{\tilde{u}_1}\right)\tilde{u}^{11}_1
$$
where $u^{11}_1 = \tilde{u}^{11}_1 n + o(n)$.

By Theorem~\ref{thm:wormald}, we have, almost surely, for every $1\leq t < t^\star n$,
$$
U^{11}_t = \left(1-\frac{t}{u_1}\right) u^{11}_1 + o(n).
$$
and $o(n) \leq 2n^{4/15}\log(n).$

For the regret, we have %\mv{***Check scalings with $n$ - any conditions on $p$?***}\jy{checked. holds for all $p\in (1/2, 1)$.}
\begin{eqnarray*}
\sum_{t=1}^{t^*n} R_t &=& \sum_{t=1}^{t^\star n} \left(1-\frac{t}{U_1}\right)U^{11}_1 + t^\star n \left(\frac{n}{2}-N_1\right) + t^\ast o(n^2)\\
&=& t^*n \left(U^{11}_1 - N_1 + \frac{n}{2}\right) - \frac{1}{2}(t^\star n)^2 \frac{U^{11}_1}{U_1} + t^\ast o(n^2)\\
&=& \frac{1}{2} (1-p)^2t^\star n^2 - \frac{1}{2}\frac{p^2}{1-(1-p)^2}(t^\star)^2 n^2 + t^\ast o(n^2)\\
&=& \frac{(1-(1-p)^2)(1-p)^4}{8p^2}n^2 + \frac{(2-p)(1-p)^2}{2p} o(n^2).
\end{eqnarray*}



\subsubsection{Proof of Lemma~\ref{lm:pa}}
\label{sec:pa}

We need to show that for any set $A$, the posterior probability that $A$ contains a type $1$ node is equal to
\begin{equation}
\pp(|A|) = \frac{|A|p}{1-p + |A|p}.
\label{equ:pa1}
\end{equation}

We will show this by induction over the cardinality of sets. We first consider the base case for sets of cardinality $2$. It suffices to consider  $(X_1, X_2)$ that are two independent Bernoulli ($p$) random variables, conditional on the event $(X_1,X_2)\neq (1,1)$. Then,
\begin{eqnarray*}
\P[(X_1, X_2)\neq (0,0) \mid (X_1, X_2) \neq (1,1)]
&=& \frac{\P[(X_1,X_2)\in \{(0,1),(1,0)\}]}{\P[(X_1,X_2)\neq (1,1)]}\\
&=& \frac{2p(1-p)}{1-p^2}\\
&=& \frac{2p}{1+p}.  
\end{eqnarray*}
This shows that (\ref{equ:pa1}) holds for the base case.

For the induction step, suppose that (\ref{equ:pa1}) holds for sets of cardinality $\leq k$. We then show that it holds for sets of cardinality $\leq k+1$. To this end, let $A\cup B$ be a set of cardinality $k+1$, with $A$ and $B$ being two disjoint sets of cardinality $\leq k$. Let $\tau(S)$ denote the event that set $S$ has at least one type $1$ item. Then, we have
\begin{eqnarray*}
\P[\tau(A\cup B) \mid \tau(A)^c \vee \tau(B)^c]
&=& \P[\tau(A) \vee \tau(B) \mid \tau(A)^c \vee \tau(B)^c ] \\
&=& \frac{\P[(\tau(A)^c \wedge \tau(B)) \vee (\tau(A)\wedge \tau(B)^c)]}{\P[\tau(A)^c \vee \tau(B)^c ]}\\
&=& \frac{(1-\P[\tau(A)])\P[\tau(B)] + \P[\tau(A)](1-\P[\tau(B)])}{1-\P[\tau(A)]\P[\tau(B)]}.
\end{eqnarray*}

Now, note
\begin{eqnarray*}
(1-\P[\tau(A)])\P[\tau(B)] &=& \frac{1}{C} p(1-p)|B|\\
\P[\tau(A)](1-\P[\tau(B)]) &=& \frac{1}{C}p(1-p)|A|
\end{eqnarray*}
and
\begin{eqnarray*}
1-\P[\tau(A)]\P[\tau(B)]
&=& \frac{1}{C}(1-p)(1-p - (|A|+|B|)p)
\end{eqnarray*}
where $C : = (1-p + |A|p)(1-p+|B|p)$.

Hence,
\begin{eqnarray*}
\P[\tau(A\cup B) \mid \tau(A)^c \vee \tau(B)^c]
= \frac{p(|A|+|B|)}{1-p+(|A|+|B|)p}
\end{eqnarray*}
which shows that (\ref{equ:pa1}) holds for $A\cup B$.

%xxx
%
%For any given integers $R$ and $T$ such that $R\leq T$, consider the Markov chain $\{(X_t, A_t)\}_{t=0}^T$, with initial value $(X_0,A_0) = (R,0)$, and transitions defined by, for $0\leq t < T$,
%\begin{eqnarray*}
%X_{t+1} &=& X_t - \xi_t\\
%A_{t+1} & = & A_t + X_t(\alpha \xi_t + \beta (1-\xi_t))
%\end{eqnarray*}
%where $\xi_t$ are independent and identically distributed Bernoulli random variables with mean $\gamma$, and $\alpha,\beta$ are positive constants.

%\begin{lemma} For the Markov chain $\{(X_t,A_t)\}_{t=0}^T$, we have
%$$
%\E[A_T] = T\left(R-\frac{1}{2}\gamma(T-1)\right)((1-\gamma)\alpha + \gamma \beta).
%$$
%\end{lemma}

%Note that
%$$
%A_T = \sum_{t=0}^{T-1}X_t(\alpha (1-\xi_t) + \beta \xi_t). 
%$$
%Hence, 
%$$
%\E[A_T] = \alpha \sum_{t=0}^{T-1}\E[(1-\xi_t)X_t] + \beta\sum_{t=0}^{T-1}\E[X_t\xi_t].
%$$

%Now, note, for $0\leq t \leq T$,
%$$
%X_t = R - \sum_{s=0}^{t-1} \xi_s.
%$$

%We have
%\begin{eqnarray*}
%\E[X_t\xi_t] &=& R\gamma - \sum_{s=0}^{t-1}\E[\xi_s \xi_t]
%= \gamma(R - t\gamma)
%\end{eqnarray*}
%and
%\begin{eqnarray*}
%\E[X_t(1-\xi_t)] &=& \E[X_t] - \E[X_t \xi_t]\\
%&=& (R-t\gamma) -(R\gamma-t\gamma^2)\\
%&=& (1-\gamma)R - t \gamma(1-\gamma)\\
%&=& (1-\gamma)(R-t\gamma). 
%\end{eqnarray*}

%Hence,
%$$
%\sum_{t=0}^{T-1}\E[\xi_t X_t] = \gamma\left( RT - \frac{1}{2}\gamma T(T-1)\right) 
%$$
%and
%$$
%\sum_{t=0}^{T-1}\E[(1-\xi_t)X_t] = (1-\gamma)\left(RT - \frac{1}{2}\gamma T(T-1)\right).
%$$
%
%It follows
%$$
%\E[A_T] = T\left(R-\frac{1}{2}\gamma(T-1)\right)((1-\gamma)\alpha + \gamma \beta).
%$$

\subsubsection{Proof of Proposition \ref{pro:epochs}}

We break $\tau$ into two parts: (a) $\tau_1$ denoting the number of steps spent examining pairs of regular matching sets, and (b) $\tau_2$ denoting the number of steps spent for examining a pair of matching sets involving a special set. 

We first upper bound the expected value of $\tau_1$. Conditional on $X_s$, $X_{s+1}$ is a binomial random variable with parameters $\lfloor X_s/2\rfloor$ and $1-\pp(2^s)^2$. Hence, for $s \geq 1$,
\begin{equation}
\E[X_{s+1}] = \E\left[\left\lfloor\frac{X_s}{2}\right\rfloor \right] (1-\pp(2^{s})^2)
\label{equ:exs}
\end{equation}
and
\begin{equation}
\E[X_1] = \frac{n}{2}(1-\pp(1)^2).
\label{equ:iexs}
\end{equation}

From (\ref{equ:exs}), we have
$$
\E[X_{s+1}] \leq \E[X_s] \frac{1-\pp(2^s)^2}{2}, \hbox{ for } s\geq 1
$$
which together with (\ref{equ:iexs}) yields
\begin{equation}
\E[X_s] \leq n\frac{1}{2^s}\prod_{i=0}^{s-1}(1-\pp(2^i)^2).
\label{equ:exs-1}
\end{equation}

Since in each super-epoch $s$ exploration of pairs from any two regular matching sets takes at most $2^{s}2^{s} = 4^s$ steps and there are at most $X_s/2$ pairs of matching sets, and there are at most $\log_2(n)$ super-epochs, we have 
\begin{equation}
\E[\tau_1] \leq \frac{1}{2}\sum_{s=1}^{\log_2(n)} 4^s\E[X_s].
\label{equ:etau1}
\end{equation}

From (\ref{equ:exs}), $\E[X_s]\leq n 2^{-s}$, hence it follows
$$
\E[\tau_1] \leq n^2.
$$

Let us define $s^* = \left\lfloor\log_2\left(c/p\right) \right\rfloor$, where $c$ is some constant such that $c > 2/(\sqrt{2}-1)$. 

From (\ref{equ:exs}) and (\ref{equ:etau1}), we have
$$
\E[\tau_1] \leq n(I(1,s^*) + I(s^*,\infty))
$$
where 
$$
I(x,y) := \sum_{s=x}^{y-1} 2^s\prod_{i=0}^{s-1}(1-\pp(2^i)^2).
$$

We first bound the term $I(1,s^*)$ as follows
$$
I(1,s^*) \leq  \sum_{s=0}^{s^*-1} 2^s \leq 2^{s^*} \leq \frac{c}{p}.
$$

We next bound the term $I(s^*,\infty)$. By definition of $s^*$, note that $s^* \geq \log_2(c/p) -1$, hence $p2^{s^*} \geq c/2$. It is readily observed that this with $c > 2/(\sqrt{2}-1)$ implies $2(1-\pp(2^{s^*})^2) < 1$.

We can write
\begin{eqnarray*}
I(s^*,\infty) &\leq & \sum_{s=s^*}^\infty (2(1-\pp(2^{s^*})^2))^s\\
&=& \frac{1}{2\pp(2^{s^*})^2-1}\left(2(1-\pp(2^{s^*})^2)\right)^{s^*}\\
&\leq & \frac{1}{2\pp(2^{s^*})^2-1}\\
& \leq & \frac{1}{2\pi c^2 - 1} \\
& = & O(1).
\end{eqnarray*}

%\mv{*** Check the requirements for $p$ for the above to hold ***}
%\jy{checked. holds for all $p\leq 1$.}

Hence, it follows
$$
\E[\tau_1] = O\left(\min\left\{\frac{n}{p},n^2\right\}\right).
$$

We next consider the number of steps $\tau_2$ spent on exploring special matching sets. We have already noted that in each super-epoch $s$, the cardinality of the special set is at most $2^{s+1}$. The special matching set can be paired with a set of cardinality at most $2^{s+1}$. Hence, in super-epoch $s$, the expected number of steps spent on examining matching sets involving the special matching set is at most $2^{s+1} 2^{s+1} = 4^{s+1}$. Now, note
\begin{eqnarray*}
\E[\tau_2] &\leq & 4\sum_{s=1}^{\log_2(n)} 4^{s}\Pr[X_s\geq 1]\\
&\leq & 4\sum_{s=1}^{\log_2(n)} 4^{s}\E[X_s]
\end{eqnarray*}
where the second inequality is by Markov's inequality. We have already shown that $\sum_{s=1}^{\log_2(n)} 4^{s}\E[X_s] = O(\min\{n/p,n^2\})$, hence, the result follows.


\subsubsection{Proof of Theorem~\ref{thm:min-reg}}

Let $X_s$ be the number of regular matching sets at the beginning of super-epoch $s$, and let $Y_s$ be the size of the special matching set. Let $Z_r$ be a random variable taking value 1 if both of the two matching sets examined in epoch $r$ contain a type 1 node, and $Z_r = 0$, otherwise.

Note that conditioning on that in epoch $r$ of super-epoch $s$ two regular matching sets are examined, we have
$$
Z_r \sim \operatorname{Ber}(\pp(2^s)^2)
$$
and, otherwise, if the examination involves the special matching set, we have
$$
Z_r \sim \operatorname{Ber}(\pp(Y_s)\pp(\xi_s))
$$
where $\xi_s=2^s$ if $X_s$ is odd, and $\xi_s = 2^{s+1}$ if $X_s$ is even and $X_{s+1}>0$.

Let $S_r$ be the number of steps in epoch $r$, $T_{s-1}$ be the first epoch of super-epoch $s$ with $T_0=0$.
Let $\tilde{R}_s$ denote the regret accumulated in super-epoch $s$.
To simplify notation, we define $K_s := \lfloor X_s/2\rfloor$.
Note that $K_s$ is the number of epochs in which two regular matching sets are explored. We also use the following definitions $p_s := \pp(2^s)$ and $q_s := 1 - p^2_s$. We show a graphic illustration of various definitions in Figure~\ref{fig:lms-algo}.

Note that there can be at most $\log_2(n)$ super-epochs.
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{LSM-algo.pdf}
    \caption{Matchings created in a super-epoch $s$.}
    \label{fig:lms-algo}
\end{figure}

Let $X^1_s$ be the number of regular matching sets at the beginning of super-epoch $s$ that contain a type 1 node.
Let $Y^1_s$ be a random variable taking value 1 if the special matching set has a type 1 node, and otherwise $Y^1_s = 0$;
if $Y_s=0$ (indicating that at the beginning of super-epoch $s$ there is no special matching set), we define $Y^1_s = 0$.
Note that
$$
X^1_s \mid X_s \sim \operatorname{Bin}(X_s, p_s)
$$
and
$$
Y^1_s \mid Y_s \sim \operatorname{Ber}(\pp(Y_s)).
$$
Let $\alpha_s$ be the conditional expected number of steps in epoch $r$, conditional on $Z_r = 0$, where $s$ is the super-epoch of epoch $r$.
Similarly, let $\beta_s$ be the conditional expected number of steps in epoch $r$, conditional on $Z_r = 1$, i.e.
$$
\alpha_s = \mathbb{E}\left[S_r | Z_r=0\right]
\text{ and }
\beta_s = \mathbb{E}\left[S_r | Z_r=1\right].
$$
Note that $\beta_s = \alpha_s / 2$.

In each step, the instantaneous regret is equal to the number of pairs of type 1 nodes that can be formed from the number of unidentified type 1 nodes. Since each regular or special matching set contains at most one type 1 node, we can express the instantaneous regret at the beginning of super-epoch $s$ as follows:
\begin{equation}
    \label{eq:R_super-epoch}
    R_{T_{s-1}} = \Bigl\lfloor \frac{X^1_s}{2} \Bigr\rfloor + Y^1_s \mathbf{1}_{\{X^1_s \text{ is odd}\}}.
\end{equation}
The instantaneous regret in epoch $T_{s-1}<r\leq T_s$ satisfies the following relation
\begin{equation}
    \label{eq:R_r}
    R_r = R_{T_{s-1}} - \sum_{i=T_{s-1}+1}^r Z_i.
\end{equation}
We will evaluate the cumulative regret of the algorithm by summing up the regret accumulated in each super-epoch. 
The regret accumulated in super-epoch $s$ can be expressed as follows:
$$
\tilde{R}_s = A_s + B_s
$$
where 
\begin{equation}
    A_s := \sum_{r=T_{s-1}+1}^{T_{s-1}+K_s} R_{r-1} S_r \label{eq:A_s}
\end{equation}
and
\begin{equation}
B_s := R_{T_{s-1}+K_s} S_{T_{s-1}+K_s+1}\left(\mathbf{1}_{\{X_s \text{ is odd}\}} + \mathbf{1}_{\{Y_s > 0\}} \mathbf{1}_{\{X_s \text{ is even}\}} + \mathbf{1}_{\{X_{s+1} > 0\}}  \right). \label{eq:B_s}
\end{equation}
Note that $A_s$ is the cumulative regret incurred in epochs of super-epoch $s$ in  which regular matching sets are examined, and $B_s$ is the regret incurred in the last epoch of super-epoch $s$ that involves examination of the special matching set, or a regular matching set of size $2^{s+1}$ and a remaining regular matching set of size $2^s$ if there is odd number of regular matching sets of size $2^s$ at the initial epoch of the super-epoch $s$.

Before proceeding with the proof, we list some basic properties of binomial distribution in the following lemma.
\begin{lemma} Assume that $X$ is a binomial random variable with parameters $n$ and $p$. Then,
\begin{enumerate}
    \item $\mathbb{E}\left[X^{2}\right]=n(n-1) p^{2}+n p$
    \item $\mathbb{E}\left[X^{3}\right]=n(n-1)(n-2) p^{3}+3 n(n-1) p^{2}+n p$.
\end{enumerate}
\end{lemma}

In the following we evaluate the expected values of $A_s$ and $B_s$ defined in (\ref{eq:A_s}) and (\ref{eq:B_s}), respectively.

\begin{lemma}
For every super-epoch $1\leq s\leq \log_2(n)$, we have
$$
\mathbb{E}[A_s] = \frac{1}{4} \left(1- \frac{1}{2}p_s\right) \left(1-\frac{1}{2}p_s^2\right) p_s\alpha_s\mathbb{E}[X_s^2] + O(n).
$$
\end{lemma}

\begin{proof}
From (\ref{eq:R_r}) and (\ref{eq:A_s}), we have $A_s = A^{(1)}_s - A^{(2)}_s$ where
\begin{equation}
A^{(1)}_s = R_{T_{s-1}} \sum_{r=T_{s-1}+1}^{T_{s-1}+K_s} S_r
\end{equation}
and
\begin{equation}
A^{(2)}_s := \sum_{r=T_{s-1}+1}^{T_{s-1}+K_s} S_r \sum_{i=T_{s-1}+1}^r Z_i.
\end{equation}

We separately consider $A^{(1)}_s$ and $A^{(2)}_s$ as follows. Note that
\begin{eqnarray*}
\mathbb{E}\left[A_{s}^{(1)} \mid T_{s-1}, X_{s}, X_{s}^{1}, Y_{s}^{1}\right] &=& \mathbb{E}\left[R_{T_{s-1}} \mid X_{s}, X_{s}^{1}, Y_{s}^{1}\right]
= \mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} S_{r} \mid T_{s-1}, X_{s}, X_{s}^{1}\right].
\end{eqnarray*}

By (\ref{eq:R_super-epoch}), we have 
$$
\mathbb{E}\left[R_{T_{s-1}} \mid X_{s}, X_{s}^{1}, Y_{s}^{1}\right]=\left\lfloor\frac{X_{s}^{1}}{2}\right\rfloor+Y_{s}^{1} \1_{\{X^1_s \text{ is odd}\}}
$$
We can write 
\begin{equation}
    \mathbb{E}\left[A^{(1)}_s \mid T_{s-1} X_{s}, X_{s}^{1}, Y_{s}^{1}\right]=\left( \left\lfloor\frac{X_{s}^{1}}{2}\right\rfloor+Y_{s}^{1} \1_{\{X^1_s \text{ is odd}\}} \right) N_s
\end{equation}
where 
$$
N_s := \mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} S_{r} \mid T_{s-1}, X_{s}, X_{s}^{1}\right].
$$
We next evaluate $N_{s}$. Let us define $K_{s}^{11}$ to be the number of epochs in super-epoch $s$ in which two regular matching sets are examined such that both have a value 1 node, i.e. $K_{s}^{11}:=$ $\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} Z_{r} .$ Then, note
\begin{eqnarray*}
N_{s} &=& \beta_{s} \mathbb{E}\left[K_{s}^{11} \mid X_{s}, X_{s}^{1}\right]+\alpha_{s} \mathbb{E}\left[K_{s}-K_{s}^{11} \mid X_{s}, X_{s}^{1}\right] \\
&=& \alpha_s \left(K_s - \frac{1}{2} \mathbb{E}[K^{11}_s \mid X_s, X^1_s]\right).
\end{eqnarray*}

This requires evaluating the expected number of pairs of 1-1 matching sets, given that there are $X_s$ matching sets in which $X^1_s$ matching sets contain a type 1 node.
Hence, we have
$$
\mathbb{E}\left[K^{11}_s \mid X_s, X^1_s\right] = K_s \left(\frac{X^1_s}{X_s}\right)^2
$$
and 
$$
N_s = \alpha_s K_s \left[1 - \frac{1}{2}  \left(\frac{X^1_s}{X_s}\right)^2\right] = \alpha_s \left\lfloor \frac{X_s}{2} \right\rfloor \left[1 - \frac{1}{2}  \left(\frac{X^1_s}{X_s}\right)^2\right].
$$
Note that 
\begin{equation*}
\begin{aligned}
\mathbb{E}\left[ \left\lfloor\frac{X_{s}^{1}}{2}\right\rfloor \left\lfloor \frac{X_s}{2} \right\rfloor \left[1 - \frac{1}{2}  \left(\frac{X^1_s}{X_s}\right)^2\right] \mid X_{s}\right] 
&= \frac{X_s}{4} \mathbb{E}\left[ X^1_s - \frac{(X^1_s)^3}{2X_s^2} \mid X_s \right]\\
&= \frac{X_s \mathbb{E}[X^1_s \mid X_s]}{4} - \frac{\mathbb{E}[(X^1_s)^3 \mid X_s]}{8X_s} \\
&= \frac{1}{4}p_s X_s^2 - \frac{1}{8}p_s^3 X_s^2 + O(n)
\end{aligned}
\end{equation*}
and
\begin{equation*}
\mathbb{E}\left[A_{s}^{(1)} \mid T_{s-1}, X_{s}, X_{s}^{1}, Y_{s}^{1}\right]=\left(\left\lfloor\frac{X_{s}^{1}}{2}\right\rfloor+Y_{s}^{1} 1_{\left\{X_{s}^{1} \text { odd }\right\}}\right) N_{s}.
\end{equation*}
It follows that we have
$$
\mathbb{E}\left[A_{s}^{(1)} \right]
= \frac{1}{4} p_s \left(1- \frac{1}{2}p_s^2\right) \alpha_s\mathbb{E}[X_s^2] + O(n).
$$

Next, we upper bound the expected value of $A_s^{(2)}$. Note that
\begin{equation*}
\begin{aligned}
\mathbb{E}\left[A_{s}^{(2)}\right] &=\mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} S_{r} \sum_{i=T_{s-1}+1}^{r} Z_{i}\right] \\
&=\mathbb{E}\left[\mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} S_{r} \sum_{i=T_{s-1}+1}^{r} Z_{i} \mid T_{s-1}, K_{s}\right]\right] \\
&= \mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} \mathbb{E}\left[\left(\alpha_{s}\left(1-Z_{r}\right)+\beta_{s} Z_{r}\right) \sum_{i=T_{s-1}+1}^{r} Z_{i} \mid T_{s-1}, K_{s}\right]\right] \\
& = \mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} \mathbb{E}\left[ \alpha_s \sum_{i=T_{s-1}+1}^{r} Z_i - \frac{1}{2}\alpha_s Z_r \sum_{i=T_{s-1}+1}^{r} Z_i \mid T_{s-1}, K_{s}\right]\right]
\end{aligned}
\end{equation*}
where the last equality holds because $\beta_s = \alpha_s / 2$.

Evaluating
\begin{equation*}
\begin{aligned}
\mathbb{E}\left[ \sum_{i=T_{s-1}+1}^{r} Z_i \mid T_{s-1}, K_{s}\right]
&= \sum_{i=T_{s-1}+1}^{r} \mathbb{P}\left[ Z_i = 1 \right] = (r - T_{s-1}) p_s^2
\end{aligned}
\end{equation*}

and

\begin{equation*}
\begin{aligned}
\mathbb{E}\left[ Z_r \sum_{i=T_{s-1}+1}^{r} Z_i \mid T_{s-1}, K_{s}\right]
&= \mathbb{E}\left[ Z_r^2 \mid T_{s-1}, K_{s}\right] + \sum_{i=T_{s-1}+1}^{r-1} \mathbb{E}\left[ Z_r Z_i \mid T_{s-1}, K_{s}\right] \\
&= \mathbb{P}\left[ Z_i = 1 \right] + \sum_{i=T_{s-1}+1}^{r-1} \mathbb{P}\left[ Z_r = 1 \right] \mathbb{P}\left[ Z_i = 1 \right] \\
&= p_s^2 + (r - T_{s-1} - 1) p_s^4
\end{aligned}
\end{equation*}
and putting them together, we obtain
\begin{equation*}
\begin{aligned}
\mathbb{E}\left[A_{s}^{(2)}\right] &=\mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} \alpha_s (r - T_{s-1}) p_s^2 - \frac{1}{2}\alpha_s \left[ p_s^2 + (r - T_{s-1} - 1) p_s^4 \right] \right] \\
&= \mathbb{E}\left[\sum_{r=T_{s-1}+1}^{T_{s-1}+K_{s}} \alpha_s p_s^2(1-\frac{1}{2}p_s^2)(r-T_{s-1}) - \frac{1}{2}\alpha_s p_s^2(1-p_s^2) \right] \\
&= \mathbb{E}\left[ \alpha_s p_s^2(1-\frac{1}{2}p_s^2) \sum_{i=1}^{K_s} i -  \frac{1}{2}\alpha_s p_s^2(1-p_s^2) K_s \right] \\
&= \mathbb{E}\left[ \frac{1}{2}\alpha_s p_s^2(1-p_s^2) K_s^2 +  \frac{1}{4}\alpha_s p_s^4 K_s(K_s + 1) \right] \\
&= \frac{1}{8} p_s^2 \left(1-\frac{1}{2}p_s^2\right) \alpha_s \mathbb{E}[X_s^2] + O(n)
\end{aligned}
\end{equation*}
where the last equality holds because $K_s = \lfloor X_s / 2 \rfloor$.

By putting together the upper bounds for $\E[A^{(1)}_s]$ and $\E[A^{(2)}_s]$, we have 
$$
\mathbb{E}[A_s] = \frac{1}{4} \left(1- \frac{1}{2}p_s\right) \left(1-\frac{1}{2}p_s^2\right) p_s\alpha_s\mathbb{E}[X_s^2] + O(n).
$$
\end{proof}
%\endproof\Halmos

\begin{lemma}
For every super-epoch $1\leq s\leq \log_2(n)$, we have
$$
\mathbb{E}\left[B_{s}\right] \leq n 2^{s+1} p_{s}\left(1-p_{s}\right) \prod_{i=0}^{s-1} q_{i}+O(n).
$$
\end{lemma}

\begin{proof} In the last epoch of super-epoch $s$, the two matching sets are of cardinality at least $2^s$ and at most $2^{s+1}$, hence,
$$
\mathbb{E}\left[B_{s}\right] \leq \mathbb{E}\left[R_{T_{s-1}+K_{s}}\right] 4^{s+1}.
$$

Noting that $\mathbb{E}\left[R_{T_{s-1}+K_{s}}\right]=\mathbb{E}\left[R_{T_{s-1}}\right]-\mathbb{E}\left[K_{s}^{11}\right]$, we have 
%$$
%\mathbb{E}\left[R_{T_{s-1}+K_{s}}\right] \leq n p_{\mathrm{s}}\left(1-p_{\mathrm{s}}\right) \frac{1}{2^{s+1}} \prod_{i=0}^{s-1} q_{i}+O(1).
%$$
%\mv{*** Check conditions for $p$ ***}
%\jy{
$$
\mathbb{E}\left[R_{T_{s-1}+K_{s}}\right] \leq n p_{\mathrm{s}}\left(1-p_{\mathrm{s}}\right) \frac{1}{2^{s+1}} \prod_{i=0}^{s-1} q_{i}+p_{s+1}.
$$
%}
It follows
$$
\mathbb{E}\left[B_{s}\right] \leq n 2^{s+1}  p_{s}\left(1-p_{s}\right) \prod_{i=0}^{s-1} q_{i}+4p_{s+1}n^2.
$$.
\end{proof}
%\endproof\Halmos

Since the regret accumulated in super-epoch $s$ is equal to $A_s + B_s$, we have
$$
\mathbb{E}[R] \leq \sum_{s=1}^{\log _2(n)} \mathbb{E}[A_s + B_s] \leq a_{n, p} n^2 + b_{n,p} n^2 + O(n^2\log(n))
$$
and
$$
\sum_{s=1}^{\log _2(n)} p_{s+1} = \sum_{s=1}^{\log _2(n)} \frac{p 2^{s+1}}{1-p+p 2^{s+1}}
$$
where
$$
a_{n, p}=\frac{1}{4} \sum_{s=1}^{\log _{2}(n)} \left(1- \frac{1}{2}p_s\right) \left(1-\frac{1}{2}p_s^2\right) p_s\left(\prod_{i=0}^{s-1} q_{i}^{2}+\frac{1}{n} \sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=0}^{i} q_{j}\right)\left(\prod_{j=i+1}^{s-1} q_{j}^{2}\right)\right)
$$
and
$$
b_{n,p}= \frac{1}{n} \sum_{s=1}^{\log _{2}(n)}  2^{s+1}  p_{s}\left(1-p_{s}\right) \prod_{i=0}^{s-1} q_{i}.
$$

\paragraph{Properties of $a_{n,p}$ and $b_{n,p}$} Let $a_{n,p} = a_{n,p}^1 + a_{n,p}^2$ where
$$
a_{n,p}^1 := \frac{1}{4} \sum_{s=1}^{\log _{2}(n)} \left(1- \frac{1}{2}p_s\right) \left(1-\frac{1}{2}p_s^2\right) p_s \prod_{i=0}^{s-1} q_{i}^{2}
$$
and
$$
a_{n,p}^2 := \frac{1}{4}\sum_{s=1}^{\log_2(n)} \left(1-\frac{1}{2}p_s\right)\left(1-\frac{1}{2}p_s^2\right)p_s \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=0}^{i}q_j\right)\left(\prod_{j=i+1}^{s-1}q_j^2\right)
$$
and, recall that
$$
b_{n,p} = \frac{1}{n}\sum_{s=1}^{\log_2(n)} 2^{s+1} p_s(1-p_s)\prod_{i=0}^{s-1}q_i.
$$


We will use the following facts. Note that 
$$
p_i = \frac{p2^i}{1-p+p 2^i} \geq 1- \frac{1-p}{p}2^{-i}.
$$ 
The right-had side in the last inequality is positive if and only if $i\geq \log_2((1-p)/p))$. The latter condition holds for all $i\geq 0$ provided that $1/2\leq p\leq 1$.

It follows that for every $i\geq \log_2((1-p)/p)$, we have
$$
q_i = 1-p_i^2 \leq 2 \frac{1-p}{p}2^{-i}.
$$ 

We next consider three different cases depending on the value of population parameter $p$.

\paragraph{Case $1/2 < p < 1$} Note that
$$
\prod_{i=0}^{s-1} q_i^2 
\leq \prod_{i=0}^{s-1} \left(2\frac{1-p}{p}\right)^2 4^{-i} = \left(8\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-s^2}
$$
and
$$
a_{n,p}^1 \leq \frac{1}{4}\sum_{s=1}^{\log_2(n)} \prod_{i=0}^{s-1}q_i^2.
$$

Hence, it follows 
\begin{equation}
a_{n,p}^1 \leq \frac{1}{4}\sum_{s=1}^{\log_2(n)} \left(8\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-s^2}.\label{equ:cnp1}
\end{equation}

The following holds
\begin{eqnarray*}
\sum_{s=1}^{\log_2(n)} \left(8\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-s^2} &\leq & \sum_{s=1}^{\log_2(n)} \left(\frac{1}{2^{s-3}}\left(\frac{1-p}{p}\right)^2\right)^{s}\\
& \leq & 4 \left(\frac{1-p}{p}\right)^2 + 4 \left(\frac{1-p}{p}\right)^4 + \sum_{s=3}^{\log_2(n)} \left(\frac{1}{2^{s-3}}\left(\frac{1-p}{p}\right)^2\right)^{s}\\
&\leq & 4 \left(\frac{1-p}{p}\right)^2 + 4 \left(\frac{1-p}{p}\right)^4 + \min\left\{\frac{\left(\frac{1-p}{p}\right)^2}{1-\left(\frac{1-p}{p}\right)^2} , 2\right \}.
\end{eqnarray*}

Thus, we have
$$
a_{n,p}^1 \leq  \left(\frac{1-p}{p}\right)^2 + \left(\frac{1-p}{p}\right)^4 + \min\left\{\frac{1}{4}\frac{\left(\frac{1-p}{p}\right)^2}{1-\left(\frac{1-p}{p}\right)^2}, \frac{1}{2}\right\}.
$$
Note that the right hand side is $(4/3)(1-p)^2$ asymptotically for small $1-p$. We can obtain a tighter upper bound as follows.

We use the following facts to bound the sum in (\ref{equ:cnp1}). By straightforward calculus, we have 
\begin{equation}
\int_a^b e^{cx}e^{-dx^2} dx = \frac{\sqrt{\pi}}{\sqrt{d}}e^{\frac{c^2}{4d}}\left[\Phi\left(\sqrt{2d}\left(b-\frac{c}{2d}\right)\right) -\Phi\left(\sqrt{2d}\left(a-\frac{c}{2d}\right)\right)\right]
\label{equ:int}
\end{equation} 
where $\Phi(x)$ is the cumulative distribution function of a normal random variable.  

It follows
$$
\int_a^b e^{cx}e^{-dx^2} dx \leq \frac{\sqrt{\pi}}{\sqrt{d}}e^{\frac{c^2}{4d}}\Phi^c\left(\sqrt{2d}\left(a-\frac{c}{2d}\right)\right)
$$
where $\Phi^c(x) = 1-\Phi(x)$.

The following is a well known bound:
$$
\Phi^c(x) \leq \frac{1}{\sqrt{2\pi}}\frac{1}{x}e^{-\frac{x^2}{2}} \hbox{ for } x > 0.
$$

If $a - c/(2d) > 0$, we have
\begin{equation}
\int_a^b e^{cx}e^{-dx^2} dx \leq \frac{1}{2d}\frac{1}{a-\frac{c}{2d}}e^{-(da^2 - ca)}.
\label{equ:intb}
\end{equation}

Note that
\begin{eqnarray*}
\sum_{s=1}^{\log_2(n)} \left(8\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-s^2} &\leq & 4 \left(\frac{1-p}{p}\right)^2 + 4 \left(\frac{1-p}{p}\right)^4 + \left(\frac{1-p}{p}\right)^{6}\\
&& + \sum_{s=4}^{\log_2(n)} \left(\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-\frac{1}{4}s^2}.
\end{eqnarray*}

Now, by applying (\ref{equ:intb}) with $c = \log((1-p)/p)$ and $d = (1/4)\log(2)$, we have

\begin{eqnarray*} 
&& \sum_{s=4}^{\log_2(n)} \left(\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-\frac{1}{4}s^2}\\
&\leq & \int_{3}^{\log_2(n)-1} \left(\left(\frac{1-p}{p}\right)^2\right)^{x} 2^{-\frac{1}{2}x^2}dx\\
& \leq & \frac{2}{\log(2)}\frac{1}{3-4\log_2\left(\frac{1-p}{p}\right)}\exp\left(-\left(\frac{9}{4}\log(2)-6\log(2)\log_2\left(\frac{1-p}{p}\right)\right)\right)\\
&=& \frac{1}{2^{5/4}\log(2)}\frac{1}{3+4\log_2\left(\frac{p}{1-p}\right)}\left(\frac{1-p}{p}\right)^6\\
 &\leq & \frac{1}{3\cdot 2^{5/4}\log(2)}\left(\frac{1-p}{p}\right)^6.
\end{eqnarray*} 

We have shown that
\begin{eqnarray*}
\sum_{s=1}^{\log_2(n)} \left(8\left(\frac{1-p}{p}\right)^2\right)^{s} 2^{-s^2} \leq 4 \left(\frac{1-p}{p}\right)^2 + 4 \left(\frac{1-p}{p}\right)^4 + \left(1+\frac{1}{3\cdot 2^{5/4}\log(2)}\right)\left(\frac{1-p}{p}\right)^{6}.
\end{eqnarray*}

Thus, we have
$$
a_{n,p}^1 \leq  \left(\frac{1-p}{p}\right)^2 + \left(\frac{1-p}{p}\right)^4 + \frac{1}{4}\left(1+\frac{1}{3\cdot 2^{5/4}\log(2)}\right)\left(\frac{1-p}{p}\right)^{6}.
$$

Observe that the right-hand side is $(1-p)^2$ asymptotically for small $1-p$.

Next, we consider $a_{n,p}^2$ and $b_{n,p}$. Note that
\begin{eqnarray*}
a_{n,p}^2 &\leq & \frac{1}{4}\sum_{s=1}^{\log_2(n)} \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=0}^{i}q_j\right)\left(\prod_{j=i+1}^{s-1}q_j^2\right)\\
&\leq & \frac{1}{4}\sum_{s=1}^{\log_2(n)} \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}q_{i+1}\left(\prod_{j=0}^{s-1}q_j\right)\\
&\leq & \frac{1}{4}\sum_{s=1}^{\log_2(n)} \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\left(2\frac{1-p}{p} 2^{-(i+1)}\right) \left(\prod_{j=0}^{s-1}q_j\right)\\
&=& \frac{1}{4}\sum_{s=1}^{\log_2(n)} \frac{s}{n}\left(2\frac{1-p}{p}\right) \left(\prod_{j=0}^{s-1}q_j\right)\\
&\leq & \frac{1}{2}\frac{\log_2(n)}{n}\frac{1-p}{p}\sum_{s=1}^{\log_2(n)} \prod_{j=0}^{s-1}q_j
\end{eqnarray*}
and
\begin{eqnarray*}
b_{n,p} & \leq & 2 \frac{1}{n}\sum_{s=1}^{\log_2(n)} 2^{s}(1-p_s)\prod_{i=0}^{s-1} q_i
 \leq  2\frac{1}{n} \frac{1-p}{p} \sum_{s=1}^{\log_2(n)} \prod_{i=0}^{s-1} q_i.
\end{eqnarray*}

We have
\begin{eqnarray*}
\prod_{i=0}^{s-1} q_i & \leq & \prod_{i=0}^{s-1} \left(2\frac{1-p}{p}\right)2^{-i}\\
&=& \left(2\frac{1-p}{p}\right)^s 2^{-\frac{s(s-1)}{2}}\\
&=& \left((\sqrt{2})^3\frac{1-p}{p}\right)^s (\sqrt{2})^{-s^2}.
\end{eqnarray*}

Summing up, we have
\begin{eqnarray*}
\sum_{s=1}^{\log_2(n)}\prod_{i=0}^{s-1} q_i 
&\leq & 2 \left(\frac{1-p}{p}\right) + 2 \left(\frac{1-p}{p}\right)^2 + \sum_{s=3}^{\log_2(n)} \left(\frac{1}{(\sqrt{2})^{s-3}}\frac{1-p}{p}\right)^s\\
&\leq & 2\left(\frac{1-p}{p}\right) + 2 \left(\frac{1-p}{p}\right)^2 + \min\left\{ \frac{\frac{1-p}{p}}{1-\frac{1-p}{p}},\frac{1}{1-1/\sqrt{2}}\right\}.
\end{eqnarray*}

It follows that $a_{n,p}^2 = O((1-p)^2\log(n)/n)$ and $b_{n,p} = O((1-p)^2(1/n))$. 

From the above results, we conclude $a_{n,p} + b_{n,p} \leq c_{n,p}$ for some $c_{n,p}$ such that for $\gamma_n = o(1)$, we have
$$
c_{n,1-\gamma_n} \sim \gamma_n^2 \hbox{ for large } n.
$$

\paragraph{Case $p \leq c/n$, for a constant $c > 0$} Note that
$$
a_{n,p}^1 \leq \frac{1}{4}\sum_{s=1}^{\log_2(n)} p_s
$$
$$
a_{n,p}^2 \leq \frac{1}{2}\sum_{s=1}^{\log_2(n)} p_s 
$$
and
$$
b_{n,p} \leq 2\sum_{s=1}^{\log_2(n)} p_s.
$$

We will use the following basic fact
\begin{eqnarray*}
\int_a^b \frac{p 2^s}{1-p+p2^s}ds &=& \frac{1}{\log(2)}\int_{2^a}^{2^b} \frac{p}{1-p+pz}dz\\
&=& \frac{1}{\log(2)}\int_{1-p+p2^a}^{1-p+p2^b}\frac{dy}{y}\\
&=& \log_2\left(\frac{1-p+p2^b}{1-p+p2^a}\right).
\end{eqnarray*}

We have the following

\begin{eqnarray*}
\sum_{s=1}^{\log_2(n)} p_s &=& \sum_{s=1}^{\log_2(n)} \frac{p2^s}{1-p+p2^s}\\
&\leq & \int_1^{\log_2(n)+1} \frac{p 2^s}{1-p+p2^s}ds\\
&=& \log_2\left(\frac{1-p+2np}{1+p}\right)\\
&\leq & \log_2(1+2np)\\
&\leq & \log_2(1+2c).
\end{eqnarray*}

Hence, it follows that $a_{n,p}^1 = O(1)$, $a_{n,p}^2 = O(1)$, and $b_{n,p} = O(1)$.

\paragraph{Case $\omega(1/n) \leq p < 1/2$} We first upper bound $a_{n,p}^1$. Let $c$ be a fixed constant $0 < c < 1$ and $s^* = (1/2)\log_2(1/c) + \log_2((1-p)/p)$. Note that
\begin{eqnarray*}
a_{n,p}^1 &\leq & 
\frac{1}{4}\sum_{s=1}^{\log_2(n)} p_s \prod_{i=0}^{s-1}q_i^2
\leq \frac{1}{4}\sum_{s=1}^{s^*} p_s + \frac{1}{4}\sum_{s=s^*+1}^{\log_2(n)} \prod_{i=s^*}^{s-1}q_i^2.
\end{eqnarray*}

Note that
\begin{eqnarray*}
\prod_{i=s^*}^{s-1} q_i^2 & \leq &  \prod_{i=s^*}^{s-1}\left(2\frac{1-p}{p}\right)^2 4^{-i}\\
& = & \left(4\left(\frac{1-p}{p}\right)^2\right)^{s-s^*} 2^{-((s-1)s-(s^*-1)s^*)}\\
& = & \left(8\left(\frac{1-p}{p}\right)^2\right)^{s-s^*} 2^{-(s^2-s^*)}\\
&=& \left(\frac{1}{2^{s+s^*-3}}\left(\frac{1-p}{p}\right)^2\right)^{s-s^*}.
\end{eqnarray*}

For every $s\geq s^*+1$, we have
\begin{eqnarray*}
\frac{1}{2^{s+s^*-3}}\left(\frac{1-p}{p}\right)^2 & \leq & \frac{1}{2^{2(s^*-1)}}\left(\frac{1-p}{p}\right)^2 = c.
\end{eqnarray*}

Hence, it follows
$$
\sum_{s=s^*+1}^{\log_2(n)} \prod_{i=s^*}^{s-1}q_i^2 \leq \sum_{s=s^*+1}^{\log_2(n)} c^s \leq \frac{1}{1-c}.
$$

Now, note also
\begin{eqnarray*}
\sum_{s=1}^{s^*} p_s & = & \sum_{s=1}^{s^*} \frac{p2^s}{1-p+p2^s}\\
&\leq & \int_1^{s^*+1} \frac{p2^s}{1-p+p2^s}ds\\
&=& \log_2\left(\frac{1-p+p 2^{s^*+1}}{1+p}\right)\\
&\leq & \log_2(1+ p 2^{s^*+1})\\
&\leq & \log_2\left(1+2/\sqrt{c} \right).
\end{eqnarray*}

We have thus shown that
$$
a_{n,p}^1 \leq \frac{1}{4}\left(\log_2\left(1+\frac{1}{\sqrt{c}}\right)+\frac{1}{1-c}\right).
$$

We next consider $a_{n,p}^2$. Fix a constant $0 < c < 1$ and let $s^* = \log_2(1/c) + \log_2((1-p)/p) + 1$.

\begin{eqnarray*}
A &:=& \sum_{s=1}^{s^*} \left(1-\frac{1}{2}p_s\right)\left(1-\frac{1}{2}p_s^2\right)p_s \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=0}^{i}q_j\right)\left(\prod_{j=i+1}^{s-1}q_j^2\right)\\
&\leq & \sum_{s=1}^{s^*} p_s \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\\
&\leq & \sum_{s=1}^{s^*} p_s \frac{1}{n} 2(2^s-1)\\
&\leq & 2\frac{2^{s^*}-1}{n}\sum_{s=1}^{s^*} p_s\\
&\leq & 2\frac{2^{s^*}-1}{n} \log_2\left(\frac{1-p+p2^{s^*+1}}{1+p}\right)\\
&\leq & 2\frac{2^{s^*}-1}{n} \log_2\left(1+p2^{s^*+1}\right)
\end{eqnarray*}

\begin{eqnarray*}
B &:=& \sum_{s=s^*+1}^{\log_2(n)} \left(1-\frac{1}{2}p_s\right)\left(1-\frac{1}{2}p_s^2\right)p_s \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=0}^{i}q_j\right)\left(\prod_{j=i+1}^{s-1}q_j^2\right)\\
&\leq & \sum_{s=s^*+1}^{\log_2(n)} \frac{1}{n}\sum_{i=0}^{s-1} 2^{i+1}\left(\prod_{j=s^*}^{s-1}q_j\right)\\
&\leq & 2 \sum_{s=s^*+1}^{\log_2(n)} \left(\prod_{j=s^*}^{s-1}q_j\right).
\end{eqnarray*}

Note that
\begin{eqnarray*}
\prod_{i=s^*}^{s-1} q_i & \leq &  \prod_{i=s^*}^{s-1}\left(2\frac{1-p}{p}\right) 2^{-i}\\
& = & \left(2\left(\frac{1-p}{p}\right)\right)^{s-s^*} 2^{-\frac{1}{2}((s-1)s-(s^*-1)s^*)}\\
& = & \left((\sqrt{2})^3\left(\frac{1-p}{p}\right)\right)^{s-s^*} (\sqrt{2})^{-(s^2-s^*)}\\
&=& \left(\frac{1}{(\sqrt{2})^{s+s^*-3}}\left(\frac{1-p}{p}\right)\right)^{s-s^*}.
\end{eqnarray*}

For every $s\geq s^*+1$, we have
$$
\frac{1}{(\sqrt{2})^{s+s^*-3}}\left(\frac{1-p}{p}\right) \leq \frac{1}{(\sqrt{2})^{2(s^*-1)}}\left(\frac{1-p}{p}\right) = c.
$$

It follows that 
$$
B \leq 2 \frac{1}{1-c}
$$
and 
\begin{eqnarray*}
A &\leq & 2 \frac{2\frac{1}{c}\frac{1-p}{p}-1}{n}\log_2\left(1+4(1-p)\frac{1}{c}\right)\\
&\leq & \frac{4}{c}\frac{1}{pn}\log_2\left(1+\frac{4}{c}\right).
\end{eqnarray*}

We have thus shown that
$$
a_{n,p}^2 \leq \frac{1}{c}\frac{1}{pn}\log_2\left(1+\frac{4}{c}\right) + \frac{1}{2}\frac{1}{1-c} = \frac{1}{2} \frac{1}{1-c} + o(1).
$$

Finally, we consider $b_{n,p}$. This is similar to bounding $a_{n,p}^2$ as note
\begin{eqnarray*}
b_{n,p} &\leq & \frac{1}{n}\sum_{s=1}^{s^*} 2^{s+1}p_s + \frac{1}{n}\sum_{s=s^*+1}^{\log_2(n)} 2^{s+1} \prod_{i=s^*}^{s-1}q_i\\
&\leq & \frac{2(2^{s^*}-1)}{n}\sum_{s=1}^{s^*} p_s + 2 \sum_{s=s^*+1}^{\log_2(n)} \prod_{i=s^*}^{s-1}q_i.
\end{eqnarray*}


By the bounds established for $a_{n,p}^2$, we have 
$$
b_{n,p} \leq \frac{1}{c}\frac{1}{pn}\log_2\left(1+\frac{4}{c}\right) + \frac{1}{2}\frac{1}{1-c} = \frac{1}{2} \frac{1}{1-c} + o(1).
$$

\subsubsection{Proof of Theorem~\ref{thm:aff}}
\label{sec:aff}

Let $X_0$ be the number of node pairs of $0$-$1$ type in $M_1$. Note that
$$
\mu(M^*) = \frac{n}{2} - 1_{\{X_0 \hbox{ is odd}\}}.
$$
Note also that in a round in which the matching is such that the number of $0$-$1$ type node pairs is equal to $x$, the expected reward is $n/2 - x$. 

Let $r_x$ denote the expected instantaneous regret accrued while the number of $0$-$1$ type node pairs is equal to $x\leq x_0$ conditional on the number of $0$-$1$ type node pairs in $M_1$ equal to $x_0$. Then, note
$$
r_x = \frac{3}{2}\left(x - 1_{\{x_0 \hbox{ is odd }\}}\right).
$$

It follows
\begin{eqnarray*}
\lim_{T\rightarrow \infty}R^\alg(T) &=&  \E\left[\sum_{i=0}^{\lfloor X_0/2\rfloor -1} r_{X_0-2i}\right]\\ 
&=& \frac{3}{2}\E\left[\sum_{i=0}^{\lfloor X_0/2\rfloor -1}(X_0 -2i - 1_{\{X_0 \hbox{ is odd}\}})\right]\\
&=& \frac{3}{2}\left(\E\left[\lfloor \frac{X_0}{2}\rfloor \left(X_0 - 1_{\{X_0 \hbox{ is odd}\}}\right)\right] - \E\left[\lfloor\frac{X_0}{2}\rfloor\left(\lfloor\frac{X_0}{2}\rfloor-1\right)\right]\right)\\
&\sim & \frac{3}{8}\E[X_0^2] \hbox{ for large } n\\
&\sim & \frac{3}{8} [p(1-p)]^2 n^2 \hbox{ for large } n.
\end{eqnarray*}


\subsubsection{Proof of Lemma~\ref{lm:alpha-function}}
\label{sec:alpha-function}

\subsubsection{Proof of Lemma~\ref{lm:xor-gb}} 
\label{sec:xor-gb}

The statement clearly holds when the collection consists of two matching sets. For a collection of three or more matching sets, it suffices to show that for arbitrary three matchings sets from the collection, the expected reward is largest by re-matching matches from two matching sets of smallest size from these three matching sets. Let $A$, $B$, and $C$ be three arbitrary disjoint sets of matches, and let $a=|A|$ and $b=|B|$, and $c=|C|$. Let 
$$
f(x,y) = \pi(x)(1-\pi(y)) + (1-\pi(x))\pi(y)
$$
where for positive integers $x$ and $y$, and recall $\pi(z) = p^{2z}/(p^{2z}+(1-p)^{2z})$.

Assume that $b\leq c$, then we claim that $f(a,b)\geq f(a,c)$.

Note that $f(a,y)$ is a convex combination of points $\pi(a)$ and $1-\pi(a)$ with respective weights $1-\pi(y)$ and $\pi(y)$. To show that $f(a,b)\geq f(a, c)$, it suffices to show that $(\pi(b),1-\pi(b))$ puts larger weight on the largest value between $\pi(a)$ and $1-\pi(a)$, than $(\pi(c), 1-\pi(c))$. 

Consider first the case $0\leq p\leq 1/2$. Then, we have $1-\pi(a)\geq \pi(a)$. Hence, we need to show that $\pi(b)\geq \pi(c)$. This indeed holds as it can be readily observed that $\pi(y)$ is decreasing in $y$. For the case $1/2<p\leq 1$, we have $\pi(a)\geq 1-\pi(a)$, hence, we need to show that $\pi(b)\leq \pi(c)$. This indeed holds as it can be readily observed that $\pi(y)$ is increasing in $y$.

By the above arguments, for any set $A$, it is optimal to create matches between $A$ and a set of smallest size between $B$ and $C$. Hence, a set of the smallest size among $A$, $B$ and $C$ is contained in this pair of sets. By the claim established above and taking $A$ to be the smallest set among $A$, $B$ and $C$, it follows that a pair of sets that maximizes $f(|U|,|V|)$ over $U,V\in \{A,B,C\}$  such that $U\neq V$ are two sets among $A$, $B$ and $C$ of smallest size.

%The expected reward of re-matching two pairs from $A$ is $$2\pi(|A|)(1-\pi(|A|)).$$
%The expected reward of re-matching two pairs from $A$ and $B$, respectively, is
%$$
%\pi(|A|)(1-\pi(|B|)) + (1-\pi(|A|))\pi(|B|).
%$$
%The proof follows by noting that, for every $p\in [0,1]$, 
%\begin{eqnarray*}
%&& 2\pi(|A|)(1-\pi(|A|)) - \left[\pi(|A|)(1-\pi(|B|)) + (1-\pi(|A|))\pi(|B|)\right] \\
%&=& 2 \frac{p^{2a}}{p^{2a} + (1-p)^{2a}} \frac{(1-p)^{2a}}{p^{2a} + (1-p)^{2a}} -  \frac{p^{2a}}{p^{2a} + (1-p)^{2a}}  \frac{(1-p)^{2b}}{p^{2b} + (1-p)^{2b}} - \frac{(1-p)^{2a}}{p^{2a} + (1-p)^{2a}}  \frac{p^{2b}}{p^{2b} + (1-p)^{2b}} \\
%&=& \frac{\left[p^{2b-2a}-(1-p)^{2b-2a}\right]\left[p^{2a}-(1-p)^{2a}\right]p^{2a}(1-p)^{2a}}{\left[ p^{2a} + (1-p)^{2a}  \right]^2 \left[ p^{2b} + (1-p)^{2b} \right]} \geq 0.
%\end{eqnarray*}

\subsubsection{Proof of Lemma~\ref{lm:cesop1}}

Denote by $k$ the number of value $1$ nodes. Let $M^\ast$ be an optimal matching and let $n_{i,j}$ denote the number of $i-j$ pairs in this matching. Then, we can write $\mu(M^\ast) = n_{0,1} + 2^{1/a}n_{1,1} = 2^{1/a-1} k - \left(2^{1/a-1} - 1\right)n_{1,0}$.
Consider a matching $\bar{M}$ which prioritizes pairing of same types, i.e. $\mu(\bar{M})= 2^{1/a}\lfloor k/2 \rfloor + \1_{k \text{ is odd}}$.
Note that $\mu(M^\ast) \geq \mu(\bar{M})$, hence
\begin{equation*}
    \begin{split}
        2^{1/a-1} k - \left(2^{1/a-1} - 1\right)n_{0,1} &\geq 2^{1/a}\lfloor k/2 \rfloor + \1_{k \text{ is odd}} = 2^{1/a-1} k - \left(2^{1/a-1} - 1\right) \1_{k \text{ is odd}}\\
    \end{split}
\end{equation*}
which yields $n_{0,1} \leq \1_{k \text{ is odd}}\leq 1$.

Conversely, assume that $M^\ast$ is an optimal matching such that it contains two $0$-$1$ pairs. Then we can construct a new matching $\tilde{M}$ which replaces the two $0$-$1$ pairs in $M^\ast$ with $1$-$1$ and $0$-$0$ pairs and $\mu(\tilde{M}) - \mu(M^\ast) = \f(1,1)+\f(0,0) - 2\f(0,1) = 2^{1/a} - 2 > 0$, which is a contradiction of the assumption that $M^\ast$ is an optimal matching.

\subsubsection{Proof of Theorem~\ref{thm:ces1}}
\label{app:ces1}

Let $N^{01}$ be the number of nodes in $0$-$1$ matches of the initial random matching. 

The algorithm iterates through super-rounds $s$ from $2$ to $\lfloor N^{01}/2\rfloor + 1$. In each super-round, it selects two matched pairs from the set containing $0$-$1$ type matches and rematches these two pairs. Each super-round consists of one or two rounds. At the end of a super-round, two new matches of $0$-$0$ and $1$-$1$ type are created. 

Let $\tilde{R}_s$ denote the regret accrued in super-round $s$. The expected regret satisfies
$$
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) = \E\left[\sum_{s=1}^{\lfloor N^{01}/2\rfloor +1} \tilde{R}_s\right].
$$

With a slight abuse of notation, let $R_s$ denote the instantaneous regret in the last round of super-round $s$. Then, for $s > 1$,
\begin{equation}
\tilde{R}_{s} = R_{s-1} - (2^{1/a}-2) + \xi_{s-1}
\label{equ:tildeR}
\end{equation}
where $\P[\xi_s = R_s] = \P[\xi_s = 0] = 1/2$.

By taking expectation on both sides in equation (\ref{equ:tildeR}), we have, for $s > 1$,
$$
\E[\tilde{R}_s] = \frac{3}{2}\E[R_{s-1}] - (2^{1/a}-2).
$$

Note that
$$
\tilde{R}_1 = R_1 = (2^{1/a}-2) \left\lfloor\frac{N^{01}}{2}\right\rfloor
$$
and, for $s > 1$,
$$
R_s = R_{s-1} - (2^{1/a}-2).
$$
Thus, for $s\geq 1$,
$$
R_s = (2^{1/a}-2)\left(\left\lfloor\frac{N^{01}}{2}\right\rfloor - (s-1)\right).
$$

Summing up, we have
\begin{eqnarray*}
\E\left[\sum_{s=1}^{\lfloor N^{01}/2\rfloor +1} \tilde{R}_s\right]
& = & \E[R_1] + \frac{3}{2}\E\left[\sum_{s=1}^{\lfloor N^{01}/2\rfloor} R_s \right] - (2^{1/a}-2) \E\left[\left\lfloor\frac{N^{01}}{2}\right\rfloor\right]\\
&=& \frac{3}{2}\E\left[\sum_{s=1}^{\lfloor N^{01}/2\rfloor} R_s \right]\\
&=& \frac{3}{4}(2^{1/a}-2) \E\left[\left\lfloor\frac{N^{01}}{2}\right\rfloor\left(\left\lfloor\frac{N^{01}}{2}\right\rfloor+1\right)\right].
\end{eqnarray*}

Since $N^{01}/n \sim 2p(1-p)$ for large $n$, it follows
$$
\E\left[\sum_{s=1}^{\lfloor N^{01}/2\rfloor +1} \tilde{R}_s\right] \sim \frac{3}{4}(2^{1/a}-2)[p(1-p)]^2 n^2 \hbox{ for large } n.
$$

\subsubsection{Proof of Lemma~\ref{lm:cesopt2}}

Denote by $k$ the number of value $1$ nodes.
Let $M^\ast$ be an optimal matching and let $n_{i,j}$ denote the number of $i-j$ pairs in this optimal matching. Then $\mu(M^\ast) = n_{0,1}\f(0,1) + n_{1,1}\f(1,1) = k - \left(2 - 2^{1/a}\right)n^{11} = (1-2^{1/a -1})n + (2^{1/a}-1)k - (2-2^{1/a})n_{0,0}$. Denote by $\tilde{M}$ a matching which prioritizes the $0$-$1$ pairs. First, consider the case $k< n/2$, then $\mu(\tilde{M}) = k \f(0,1)=k$. Note that $\mu(M^\ast)\geq \mu(\tilde{M})$, hence $n_{1,1}=0$. Second, consider the case when $k\geq n/2$, then $\mu(\tilde{M}) = (k-n/2)\f(1,1) + (n-k)\f(0,1)=(1-2^{1/a-1})n + (2^{1/a}-1)k$.
Note that $\mu(M^\ast)\geq \mu(\tilde{M})$, hence $n_{0,0}=0$. We have thus shown that in an optimal matching either $n_{0,0} = 0$ or $n_{1,1} = 0$.

Conversely, assume that an optimal matching $M^\ast$ contains one $0$-$0$ pair and one $1$-$1$ pair. Then we can construct a new matching $M^\prime$ which replaces the $0$-$0$ pair and the $1$-$1$ pair in $M^\ast$ with two $0$-$1$ pairs and $\mu(M^\prime) - \mu(M^\ast) =2\f(0,1)-\f(1,1)-\f(0,0) = 2 - 2^{1/a} > 0$, which is a contradiction of the assumption that $M^\ast$ is an optimal matching.

\subsubsection{Proof of Theorem~\ref{thm:ces2}}
\label{app:ces2}

Let $N^{00}$ and $N^{11}$ be the number of matches in the initial random matching known to be of type $0$-$0$ and $1$-$1$, respectively.

The instantaneous regret satisfies 
$$
R_1 = (2-2^{1/a})(N^{00}\wedge N^{11})
$$
and, for $t > 1$,
$$
R_t = R_{t-1} - (2-2^{1/a})\ind_{\{R_{t-1} > 0\}}.
$$
Hence, we have
$$
R_t = (2-2^{1/a})(N^{00}\wedge N^{11}-(t-1))\ind_{\{t\leq N^{00}\wedge N^{1,1}\}}.
$$

It follows that the regret satisfies
\begin{eqnarray*}
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) 
&=& \E\left[\sum_{t=1}^{N^{00}\wedge N^{11}}R_t\right]
= (2-2^{1/a}) \E\left[\frac{N^{00}\wedge N^{11}}{2}\left(\frac{N^{00}\wedge N^{11}}{2}+1\right)\right].
\end{eqnarray*}

Now, since $N^{00}/n \sim (1-p)^2$ and $N^{11}/n \sim p^2$ for large $n$, we have
$$
\lim_{T\rightarrow \infty}\breg_{\f}^{\gb}(T) \sim \frac{1}{4}(2-2^{1/a})\min\{p,1-p\}^4 n^2 \hbox{ for large } n.
$$





